FB-4D: Spatial-Temporal Coherent Dynamic 3D Content Generation with Feature Banks

With the rapid advancements in diffusion models and 3D generation techniques, dynamic 3D content generation has become a crucial research area. However, achieving high-fidelity 4D (dynamic 3D) generation with strong spatial-temporal consistency remains a challenging task. Inspired by recent findings that pretrained diffusion features capture rich correspondences, we propose FB-4D, a novel 4D generation framework that integrates a Feature Bank mechanism to enhance both spatial and temporal consistency in generated frames. In FB-4D, we store features extracted from previous frames and fuse them into the process of generating subsequent frames, ensuring consistent characteristics across both time and multiple views. To ensure a compact representation, the Feature Bank is updated by a proposed dynamic merging mechanism. Leveraging this Feature Bank, we demonstrate for the first time that generating additional reference sequences through multiple autoregressive iterations can continuously improve generation performance. Experimental results show that FB-4D significantly outperforms existing methods in terms of rendering quality, spatial-temporal consistency, and robustness. It surpasses all multi-view generation tuning-free approaches by a large margin and achieves performance on par with training-based methods.

==> sec/0_abstract.tex <==
\begin{abstract}
Scene simulation in autonomous driving has gained significant attention because of its huge potential for generating customized data. However, existing editable scene simulation approaches face limitations in terms of user interaction efficiency, multi-camera photo-realistic rendering and external digital assets integration. 
To address these challenges, this paper introduces~\textit{ChatSim}, the first system that enables editable photo-realistic 3D driving scene simulations via natural language commands with external digital assets. To enable editing with high command flexibility,~\textit{ChatSim} leverages a large language model (LLM) agent collaboration framework. To generate photo-realistic outcomes,~\textit{ChatSim} employs a novel multi-camera neural radiance field method. Furthermore, to unleash the potential of extensive high-quality digital assets,~\textit{ChatSim} employs a novel multi-camera lighting estimation method to achieve scene-consistent assets' rendering. Our experiments on Waymo Open Dataset demonstrate that~\textit{ChatSim} can handle complex language commands and generate corresponding photo-realistic scene videos.
% including long and complex commands, highly-abstract commands and multi-round commands.

% However, previous editable simulation approaches are limited by complicated editing command execution and relatively low user operation efficiency due to their fixed editing mode design and inevitable user involvement in every intermediate trivial editing step.

 

% and the integration of external digital assets to enhance realism and flexibility. % enrich the scene's content. 





\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% Scene simulation techniques are gradually being applied to autonomous driving. The current methods for obtaining driving scene data primarily rely on real vehicle data collection, which has limitations, including: 
% (1) Lack of rare data instances, such as accidents and extreme weather conditions.
% (2) Limited control over scenes, making it challenging to edit instances within them, such as adding, removing, or replacing elements.

 
 \quad Perception~\cite{chen2015deepdriving,chen2017multi,wu2017squeezedet,chen2016monocular,caesar2020nuscenes,li2020rtm3d} is the window of an autonomous vehicle into the external environment. To ensure the robustness of the vehicle's perceptual capabilities during both training and testing phases, it necessitates the collection of high-quality perception data in substantial volumes \cite{chang2019argoverse,sun2020scalability}. However, the operation of a fleet for the acquisition of real-world data often incurs prohibitive expenses, particularly for specialized or customized requirements. For instance, in the aftermath of an accident or intervention involving an autonomous vehicle, it is imperative to test the vehicle's perception system across a spectrum of similar scenarios. While replicating such scenario data from real-world instances is nearly impossible due to the uncontrollability of actual scenes \cite{rong2020lgsvl,bergamini2021simnet}, customized scene simulation emerges as a vital and feasible alternative. It enables the precise modeling of specific conditions without high costs and logistical complexities of real-world data collection \cite{amini2020learning,yang2020surfelgan}.

\begin{figure}[t] 
\centering 
\includegraphics[width=0.47\textwidth]{imgs/teaser_update.jpg} 
\vspace{-3.5mm}
\caption{\small \textit{ChatSim} enables the editing of photo-realistic 3D driving scene simulations via language commands. 
}
\label{Fig:teaser} 
\vspace{-6mm}
\end{figure}

To effectively simulate customized driving scenes, we identify three key properties as fundamental. First, the simulation should be capable of following sophisticated or abstract demands, thereby 
facilitating the production. Second, the simulation should generate photo-realistic, view-consistent outcomes, which allow for the closest approximation to vehicle observations in real-world scenarios. Third, it should allow for the integration of external digital assets \cite{miric2019protecting,banta2016property} with their photo-realistic textures and materials while fitting the lighting conditions. This capability would unlock the potential for data expansion by incorporating a wide array of external digital assets, satisfying customized needs.

A vast array of significant works have been proposed for scene simulation, yet they fail to meet all three of these requirements. Traditional graphics engines, such as CARLA~\cite{dosovitskiy2017carla} and UE \cite{UE}, offer editable virtual environments with external digital assets, but the data realism is restricted by asset modeling and rendering qualities. Image generation based methods, such as BEVControl \cite{yang2023bevcontrol}, DriveDreamer \cite{wang2023drivedreamer}, MagicDrive \cite{gao2023magicdrive}, can generate realistic scene images based on various control signals, including BEV maps, bounding boxes and camera poses. However, they struggle to maintain view consistency and face challenges in importing external digital assets due to the absence of 3D spatial modeling. Rendering-based methods have been proposed to obtain photo-realistic and view-consistent scene simulation. Notable examples like UniSim \cite{yang2023unisim} and MARS \cite{wu2023mars} come equipped with a suite of scene-editing tools. However, these systems require extensive user involvement in every trivial editing step via code implementation, which is ineffective when performing the editing. Furthermore, while they handle vehicles in observed scenarios effectively, their inability to support external digital assets restricts opportunities for data expansion and customization.

To fulfill the identified requirements, we introduce~\textit{ChatSim}, the first system that enables editable photo-realistic 3D driving scene simulations via natural language commands with external digital assets. To use~\textit{ChatSim}, users simply engage in a conversation with the system, issuing commands through natural language without any involvement in intermediate simulation steps; see Figure \ref{Fig:teaser} for illustration.

To address complex or abstract user commands effectively,~\textit{ChatSim} adopts a large language model (LLM)-based multi-agent collaboration framework. The key idea is to exploit multiple LLM agents, each with a specialized role, to decouple an overall simulation demand into specific editing tasks, thereby mirroring the task division and execution typically founded in the workflow of a human-operated company. This workflow offers two key advantages for scene simulation. First, LLM agents' ability to process human language commands allows for intuitive and dynamic editing of complex driving scenes, enabling precise adjustments and feedback. Second, the collaboration framework enhances simulation efficiency and accuracy by distributing specific editing tasks among specialized agents, ensuring detailed and realistic simulations with improved task completion rates.

To generate photo-realistic outcomes, we propose McNeRF in ~\textit{ChatSim}, a novel neural radiance field method that incorporates multi-camera inputs, offering a broader scene rendering. This integration fully exploits camera setups on vehicles but raises two significant challenges: camera pose misalignment due to asynchronized trigger times and brightness inconsistency due to different camera exposure times. To address camera pose misalignment, McNeRF uses a multi-camera alignment to reduce extrinsic parameter noises, ensuring rendering quality. To address brightness inconsistency, McNeRF integrates the critical exposure times to recover scene radiance in HDR,  markedly mitigating the issue of color discrepancies at the intersections of two camera images with different exposure times.


% We organized agents mimicking efficient human company operation procedures in which agents automatically communicate with related colleges to obtain to-be-processed data with specific requirements. 
% To enable efficient agent collaboration and reduce the risk of hallucination, agents adhere to structured communication protocols with handovers that conform to established standards. 

To import external digital assets with their realistic textures and materials, we propose McLight, a novel multi-camera lighting estimation that blends skydome and surrounding lighting. Our skydome estimation restores accurate sun behavior with peak intensity residual connection, enabling the rendering of prominent shadows. For surrounding lighting, McLight queries McNeRF to achieve complex location-specific illumination effects, like those in the tree shade with sunlight being blocked. This significantly improves the rendering realism of the integrated 3D assets.
% \Note{sc: mention  the spatial-varting lighting effects of assets?}

% Our method jointly considers the effect of the skydome representing the effect of global illumination and the surrounding scenes representing the effect of neighboring context. Both of the estimation of skydome illumination and the surrounding scenes are integrated with multi-view inputs for a more accurate and broader scene illumination. For skydome illumination, we reconstruct the sky color, peak illuminance and peak direction through the multiview feature fusion. For surrounding appearance, we consider the object position and reconstruct the surrounding HDR light intensity by sampling rays from a high dynamic range (HDR) Neural Radiance Field (NeRF). This technique enables us to create spatially varying illumination for each object, ensuring photo-realistic rendering that accurately reflects the complex interplay of light in real-world scenarios.
 
We conduct extensive experiments on the Waymo autonomous driving dataset and show that ~\textit{ChatSim} generates photo-realistic customized perception data including dangerous corner cases according to various human language commands. Our method is compatible with mixed, highly-abstract and multi-round commands. Our method achieves SoTA performance with an improvement of 4.5\% in photo-realism with a wide-angle rendering. Moreover, we demonstrate our lighting estimation outperforms the SoTA methods both qualitatively and quantitatively, reducing the intensity error and angular error by 57.0\% and 9.9\%. 
% We also apply our simulation to augment training data to improve perception models, receiving a 1.9\% model gain.

% The main contributions of our work are:
% $\bullet$ We propose ~\textit{ChatSim}, the pioneering system that for the first time enables the editing of photo-realistic 3D driving scene simulations via language commands. ~\textit{ChatSim} supports complicated operation commands and produces photo-realistic and view-consist simulation outcomes.

% $\bullet$ In ~\textit{ChatSim}, we introduce a multi-LLM-agent collaborative framework for interpreting and executing user commands, enabling the system to systematically and accurately produce engineered solutions for complex commands.


% $\bullet$ We propose a multi-view illumination estimation to obtain more photo-realistic rendering of external digital assets, providing significant potential for flexible data expansion.

% $\bullet$ Experiments

==> sec/2_related_work.tex <==
\section{Related Work}
\vspace{-1mm}
\textbf{Scene simulation for autonomous driving.}
Current scene simulation methods can be generally divided into three categories: graphics engines, image generation, and scene rendering. Graphics engines, such as CARLA \cite{dosovitskiy2017carla}, AirSim \cite{shah2018airsim}, OpenScenario Editor \cite{openscanerio}, 51Sim-One \cite{51sim} and RoadRunner \cite{crescenzi2001roadrunner}, create a virtual world for simulating a wide range of driving scenarios. However, there exists a significant domain gap between the virtual world and reality. Image generation methods can generate realistic scene images based on different control signals, such as HD maps \cite{swerdlow2023street,gao2023magicdrive,li2023drivingdiffusion}, sketch layout~\cite{yang2023bevcontrol},  bounding boxes~\cite{li2023drivingdiffusion,wang2023drivedreamer,gao2023magicdrive}, text~\cite{li2023drivingdiffusion,wang2023drivedreamer,gao2023magicdrive,hu2023gaia} and driving actions~\cite{wang2023drivedreamer,hu2023gaia}. However, these approaches can hardly maintain scene consistency.  
To obtain a coherent driving scene, methods based on scene rendering target to reconstruct the 3D scene.  READ~\cite{li2023read} employs point clouds and uses a U-Net to render images. With the rapid development of Neural Radiance Field (NeRF)~\cite{mildenhall2021nerf, barron2021mip, barron2022mip, muller2022instant, sun2022direct, wang2023f2}, several works ~\cite{xie2023s, guo2023streetsurf, yang2023unisim, wu2023mars, ost2021neural, turki2023suds, kundu2022panoptic, ost2022neural} also exploit NeRFs
to model cars and static street backgrounds in outdoor environments. Moreover, notable examples like UniSim \cite{yang2023unisim} and MARS \cite{wu2023mars} come equipped with a suite of scene-editing tools.
However, these methods require extensive user involvement in intermediate editing steps and they fail to support external digital assets for data expansion. 
% In this work, we propose a novel neural radiance fields method that incorporates multi-camera inputs; called~McNeRF, leading to an editable scene simulation system that generates photo-realistic panorama outcomes; see a full comparison in Table~\ref{tab:method_comparison}.
In this work, we propose \textit{ChatSim} that achieves automatic simulation editing via language commands and integrates external digital assets to enhance realism and flexibility. In \textit{ChatSim}, we integrate McNeRF, a novel neural radiance field designed to leverage multi-camera inputs for high-fidelity rendering. 


\noindent\textbf{Lighting estimation.} Lighting estimation focuses on assessing the illumination conditions of a real-world environment to seamlessly integrate digital objects. Early methods \cite{lalonde2014lighting,lalonde2010sun} for outdoor environments use explicit cues like detected shadows on the ground. Recent works usually adopt learning-based approaches \cite{garon2019fast,hold2019deep,legendre2019deeplight,hold2017deep,li2018learning,zhang2019all} by predicting different lighting representations like spherical lobes \cite{boss2020two,li2018learning}, light probes \cite{legendre2019deeplight}, environment
map \cite{sengupta2019neural,somanath2021hdr}, HDR sky model \cite{hold2019deep,zhang2019all,wang2022neural} and lighting volume \cite{wang2022neural}. However, few of them consider multi-camera input, which is common for driving scenarios. In this paper, we propose a novel multi-camera lighting estimation method, McLight, combining with our McNeRF, to estimate a wider range of lighting and obtain the spatially-varying lighting effects of assets. 


% due to the limited observation perspectives of specific vehicles in the training data, using NeRF to model foreground vehicles can result in blurry and less realistic rendering effects. Moreover, these methods do not account for changes in lighting within the scene. To address the aforementioned issues, we designed a multi-view alignment mechanism, which enables the highly realistic modeling of the background and supports the generation of wide-angle images. For foreground objects, we utilize Blender to render vehicles with editable colors and types. Additionally, we designed a spatial-varying illumination estimation based on NeRF and HDR lighting to ensure photorealistic effects for the vehicles.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% \begin{table*}[]
% \scriptsize
% \begin{tabular}{c|c|ccc|ccc|c}
% \hline
% \multirow{2}{*}{Simulator}        & \multirow{2}{*}{Dimension} & \multicolumn{3}{c|}{Background}                                                    & \multicolumn{3}{c|}{Foreground Vechicles}                                                    & \multirow{2}{*}{Open-sourced} \\ \cline{3-8}
%                          &                            & \multicolumn{1}{c|}{Generative} & \multicolumn{1}{c|}{Reconstruction} & Multi-view & \multicolumn{1}{c|}{Decouplable} & \multicolumn{1}{c|}{Manipulative} & Language-controllable &                               \\ \hline
% BEVGen                   & 2D                          & \multicolumn{1}{c|}{y}          & \multicolumn{1}{c|}{n}              & y          & \multicolumn{1}{c|}{n}           & \multicolumn{1}{c|}{y}            & n                     &                               \\ 
% BEVControl               & 2D                          & \multicolumn{1}{c|}{y}          & \multicolumn{1}{c|}{n}              & y          & \multicolumn{1}{c|}{n}           & \multicolumn{1}{c|}{y}            & n                     &                               \\ 
% DriveDreamer             & 2D                          & \multicolumn{1}{c|}{y}          & \multicolumn{1}{c|}{n}              & n          & \multicolumn{1}{c|}{n}           & \multicolumn{1}{c|}{y}            & y                     &                               \\ 
% DrivingDiffusion         & 2D                          & \multicolumn{1}{c|}{y}          & \multicolumn{1}{c|}{n}              & y          & \multicolumn{1}{c|}{y}           & \multicolumn{1}{c|}{y}            & y                     & n                             \\ 
% GAIA-1                   & 2D                          & \multicolumn{1}{c|}{y}          & \multicolumn{1}{c|}{n}              & n          & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{y}            & y                     & n                             \\ 
% MagicDrive               & 2D                          & \multicolumn{1}{c|}{y}          & \multicolumn{1}{c|}{n}              & y          & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{y}            & n                     &                               \\ 
% READ                     & 3D                          & \multicolumn{1}{c|}{n}          & \multicolumn{1}{c|}{y}              & n          & \multicolumn{1}{c|}{n}           & \multicolumn{1}{c|}{n}            & n                     & y                             \\ 
% Neural Scene Graphs      & 3D                          & \multicolumn{1}{c|}{n}          & \multicolumn{1}{c|}{y}              & n          & \multicolumn{1}{c|}{y}           & \multicolumn{1}{c|}{n}            & n                     & y                             \\ 
% Neural Point Light Field & 3D                          & \multicolumn{1}{c|}{n}          & \multicolumn{1}{c|}{y}              & y          & \multicolumn{1}{c|}{y}           & \multicolumn{1}{c|}{n}            & n                     & y                             \\ 
% S-NeRF                   & 3D                          & \multicolumn{1}{c|}{n}          & \multicolumn{1}{c|}{y}              & y          & \multicolumn{1}{c|}{y}           & \multicolumn{1}{c|}{y}            & n                     & y                             \\ 
% UniSim                   & 3D                          & \multicolumn{1}{c|}{n}          & \multicolumn{1}{c|}{y}              & y          & \multicolumn{1}{c|}{y}           & \multicolumn{1}{c|}{y}            & n                     & n                             \\ 
% MARS                     & 3D                          & \multicolumn{1}{c|}{n}          & \multicolumn{1}{c|}{y}              & n          & \multicolumn{1}{c|}{y}           & \multicolumn{1}{c|}{y}            & n                     & y                             \\ 
% Ours                     & 3D                          & \multicolumn{1}{c|}{n}          & \multicolumn{1}{c|}{y}              & y          & \multicolumn{1}{c|}{y}           & \multicolumn{1}{c|}{y}            & y                     & y                             \\ \hline
% \end{tabular}
% \end{table*}

\begin{table}[t]
\center
\scriptsize
\setlength\tabcolsep{2pt}
\begin{tabular}{c|cccccccc}
\hline
Method     & \makecell{Photo-\\realistic}   & {Dim.} & \makecell{Multi-\\camera}                                                 & Editable & \makecell{External \\ assets} & Language & \makecell{Open- \\source}                             \\ \hline
CARLA~\cite{dosovitskiy2017carla} & \scalebox{0.75}{\usym{2613}}  &  3D& \checkmark 
& \checkmark & \checkmark & \scalebox{0.75}{\usym{2613}} & \checkmark \\
AirSim~\cite{shah2018airsim} & \scalebox{0.75}{\usym{2613}}  &  3D& \checkmark 
& \checkmark & \checkmark & \scalebox{0.75}{\usym{2613}}&  \checkmark \\
OpenScenario \cite{openscanerio} & \scalebox{0.75}{\usym{2613}}  &  3D& \checkmark 
& \checkmark  & \checkmark & \scalebox{0.75}{\usym{2613}}&  \checkmark \\
51Sim-One \cite{51sim}& \scalebox{0.75}{\usym{2613}}  &  3D& \checkmark 
& \checkmark & \checkmark & \scalebox{0.75}{\usym{2613}}& \scalebox{0.75}{\usym{2613}} \\
RoadRunner \cite{crescenzi2001roadrunner} & \scalebox{0.75}{\usym{2613}}  &  3D& \checkmark 
& \checkmark  & \checkmark& \scalebox{0.75}{\usym{2613}}& \checkmark \\
BEVGen~\cite{swerdlow2023street}     & \checkmark                & 2D                                      & \checkmark          & \checkmark      &  \scalebox{0.75}{\usym{2613}}       &     \scalebox{0.75}{\usym{2613}}                 &   \checkmark                            \\ 
BEVControl~\cite{yang2023bevcontrol}     & \checkmark            & 2D                          & \checkmark          & \checkmark     &  \scalebox{0.75}{\usym{2613}}      & \scalebox{0.75}{\usym{2613}}                       &      \scalebox{0.75}{\usym{2613}}                         \\ 
DriveDreamer~\cite{wang2023drivedreamer}      & \checkmark         & 2D                                   & \checkmark                     & \checkmark   &  \scalebox{0.75}{\usym{2613}}        &  \checkmark  &         \scalebox{0.75}{\usym{2613}}                            \\ 
DrivingDiffusion~\cite{li2023drivingdiffusion}    & \checkmark       & 2D                          & \checkmark                           & \checkmark   &      \scalebox{0.75}{\usym{2613}}   & \checkmark                          & \scalebox{0.75}{\usym{2613}}                             \\ 
GAIA-1~\cite{hu2023gaia}         & \checkmark            & 2D                  & \scalebox{0.75}{\usym{2613}}                  &    \checkmark    & \scalebox{0.75}{\usym{2613}}   & \checkmark                                & \scalebox{0.75}{\usym{2613}}                             \\ 
MagicDrive~\cite{gao2023magicdrive}     & \checkmark            & 2D                          & \checkmark  &\checkmark      & \scalebox{0.75}{\usym{2613}}     & \scalebox{0.75}{\usym{2613}}                               &   \scalebox{0.75}{\usym{2613}}                               \\ 
READ~\cite{li2023read}       & \checkmark                & 3D                          & \scalebox{0.75}{\usym{2613}}          & \scalebox{0.75}{\usym{2613}}         &\scalebox{0.75}{\usym{2613}}  &   \scalebox{0.75}{\usym{2613}}                                     & \checkmark                             \\ 
% Neural Scene Graphs~\cite{ost2021neural}
Neural SG~\cite{ost2021neural}    
& \checkmark    & 3D                          & \scalebox{0.75}{\usym{2613}}          & \checkmark        &\scalebox{0.75}{\usym{2613}}      & \scalebox{0.75}{\usym{2613}}                                     & \checkmark               \\ 
Neural PLF~\cite{ost2022neural}
% Neural Point Light Field~\cite{ost2022neural} 
& \checkmark  & 3D                          & \scalebox{0.75}{\usym{2613}}       & \scalebox{0.75}{\usym{2613}}          &\scalebox{0.75}{\usym{2613}}      & \scalebox{0.75}{\usym{2613}}                 & \checkmark                             \\ 
S-NeRF~\cite{xie2023s}       & \checkmark              & 3D                                 & \checkmark           & \scalebox{0.75}{\usym{2613}}    & \scalebox{0.75}{\usym{2613}}    & \scalebox{0.75}{\usym{2613}}                       & \checkmark                            \\ 
UniSim~\cite{yang2023unisim}      & \checkmark               & 3D                                 & \scalebox{0.75}{\usym{2613}}           & \checkmark    & \scalebox{0.75}{\usym{2613}}     & \scalebox{0.75}{\usym{2613}}                                    & \scalebox{0.75}{\usym{2613}}                             \\ 
MARS~\cite{wu2023mars}      & \checkmark                 & 3D                          & \scalebox{0.75}{\usym{2613}}            & \checkmark     &\scalebox{0.75}{\usym{2613}}        & \scalebox{0.75}{\usym{2613}}                 & \checkmark                              \\ 
\textbf{ChatSim (Ours)}       & \checkmark                & 3D                                   & \checkmark              & \checkmark     &\checkmark        & \checkmark                     & \checkmark                \\ \hline
\end{tabular}
\vspace{-3mm}
\caption{\small Comparison of existing and proposed methods for autonomous driving simulation.}
\label{tab:method_comparison}
\vspace{-4mm}
\end{table}

% \textbf{Rendering} NeRF~\cite{mildenhall2021nerf}, F2NeRF~\cite{wang2023f2}, DVGO~\cite{sun2022direct}, Mip-NeRF~\cite{barron2021mip}, Mip-NeRF360~\cite{barron2022mip}, Instant-NGP~\cite{muller2022instant}, \textbf{Autonomous Driving scene rendering}
% S-NeRF~\cite{xie2023s}, READ~\cite{li2023read}, StreetSurf~\cite{guo2023streetsurf}, UniSim~\cite{yang2023unisim}, Urban Radiance Field~\cite{Rematas_2022_CVPR}, MARS~\cite{wu2023mars}, Neural Scene Graphs~\cite{ost2021neural}, SUDS~\cite{turki2023suds}, Panoptic Neural Field~\cite{kundu2022panoptic}, GeoSim~\cite{chen2021geosim},Neural Point Light Field~\cite{ost2022neural},  \textbf{Illumination Estimation}: Zian's Neural Light Field Estimation~\cite{wang2022neural}, Zian's Inverse Rendering~\cite{wang2023neural}

% \textbf{Generation}
% GAIA-1~\cite{hu2023gaia}, DriveDreamer~\cite{wang2023drivedreamer}, DrivingDiffusion~\cite{li2023drivingdiffusion},
% MagicDrive~\cite{gao2023magicdrive}, BEVGen~\cite{swerdlow2023street}, BEVControl~\cite{yang2023bevcontrol}

\noindent\textbf{Large language model and collaborative framework.}
Large Language Models (LLMs) are AI systems trained on extensive data to understand, generate, and respond to human language. GPT \cite{llm_gpt3} is a pioneering work to generate human-like content. The following updated versions GPT-3.5 \cite{chatgpt} and GPT-4 \cite{llm_gpt4}, provide more intelligent capabilities like chatting, browsing and coding. Notable other large language models include InstructGPT \cite{ouyang2022training}, LLaMA \cite{touvron2023llama} and PaLM \cite{chowdhery2022palm,anil2023palm}. Based on LLM, many works \cite{wang2023unleashing,du2023improving,zhuge2023mindstorms,hao2023chatllm,akata2023playing} improve the problem-solving abilities by integrating communication among multiple agents. \cite{hong2023metagpt} and \cite{wu2023autogen} define a group of well-organized agents to form operating procedures with conversation and code programming. 
In this paper, we exploit the power of collaborative LLM agents in simulation for 
autonomous driving, enabling the various editing of 3D scenes via language commands.

% Despite the success of LLMs and their collaboration, exploiting the power of collaborative LLMs in autonomous driving remains an open challenge, as the inputs and outputs of autonomous systems are not languages. 

% In this paper, we propose a framework that leverages the collaboration among multiple LLMs to fulfill user-specific scene editing requirements.

% Large Language Models (LLMs) are artificial intelligence systems trained on Internet-scale data to understand and generate human-like text, showcasing remarkable abilities in natural language processing. GPT \cite{llm_gpt3} is a pioneering work that proposed the Generative Pre-trained Transformer to tackle language understanding and generation problems. The following versions GPT-3.5 and GPT-4 \cite{llm_gpt4} demonstrated impressive chatting and reasoning ability. LLaMA and LLaMA 2 \cite{llm_llama, llm_llama2} are open-source foundation language models. To better harness the capabilities of LLMs, InstructGPT \cite{llm_instructgpt} proposed to train LLMs to follow instructions with human feedback. \cite{llm_cot} proposed chain-of-thought prompting to enhance the reasoning ability of LLMs. ReAct \cite{llm_react} exploited the synergy of reasoning and acting in LLMs. These methods have bolstered the language understanding and decision-making capabilities of LLMs. 

% Despite the success of LLMs in language understanding, exploiting the power of LLMs in autonomous driving remains an open challenge, as the inputs and outputs of autonomous systems are not languages. 
% Large language models (LLMs) offer a promising approach to capturing and representing compressed knowledge and human experiences, effectively projecting them into the realm of language. LLMs have consistently demonstrated remarkable performance that extends well beyond traditional language processing domains. They possess the capability to tackle intricate tasks that were previously reserved for specialized algorithms or human experts. These tasks encompass diverse areas such as mathematical reasoning, medicine, and planning.

% The versatility and power of LLMs make them a valuable tool for addressing a wide range of challenging problems, leveraging their comprehensive understanding of language and their ability to process and reason with vast amounts of information.


==> sec/3_method.tex <==

\section{Collaborative LLM-Agents for Editing}
\vspace{-1mm}
\label{sec:3}
 % The overall architecture of the proposed ChatSim is illustrated in Fig.xx. It receives user input of commands with advanced, complex semantics, and ultimately generates edited autonomous driving scene images or videos that meet user requirements. The entire system can be divided into two parts: \textbf{Agent of project manager}, which can receive complex user commands and break them down into multiple sequentially executable sub-commands to distribute to subsequent agents. \textbf{Technique Agents}, which consists of several functional agents collaborating with each other, responsible for different technical segments in the simulation process. Specifically, we designed 6 agents to provide technical support, including Tech Agent for (1) View Adjustment (2) Vehicle Deleting (3) 3D Asset Management (4) Vehicle Motion (5) Background Rendering (6) Foreground Rendering. All these agents will be elaborated in Sec~\ref{subsec:tech_agent_design} in detail. Notably, all agents are equipped with LLMs, enabling communication and collaboration amongst agents through natural language, as well as interaction with users.
\quad
The \textit{ChatSim} system analyzes specific user commands and returns a video that meets customized needs; see Figure \ref{Fig:overview}. Since user commands could be abstract and sophisticated, it requires the system to have flexible task-handling ability. Directly applying a single LLM agent struggles with multi-step reasoning and cross-referencing. To address this, we design a series of collaborative LLM agents, where each agent is responsible for a unique aspect of the editing task. 
%This collaborative design assigns clear, specific roles to each agent and systematically produces engineered solutions to meet various commands.
% Subsequent sections will detail the roles and implementations of agents. 
% for more information, please refer to the appendix.

\begin{figure*}[t] 
\centering 
\includegraphics[width=0.99\textwidth]{imgs/method.pdf} 
\vspace{-3mm}
\caption{\small \textbf{\textit{ChatSim} system overview.} The system exploit multiple collaborative LLM agents with specialized roles to decouple an overall demand into specific editing tasks. Each agent equips an LLM and corresponding role functions to interpret and execute its specific tasks.   }
\label{Fig:overview} 
\vspace{-4mm}
\end{figure*}

% \textbf{Agent of Project Manager} is a pure LLM agent. It parses user's requirements and breaks them down for each Technique Agent. 

% In practical scenarios, user requirements often tend to be complex, mixed, and abstract. These instructions are often challenging to be directly processed and executed by a single agent. The role of the Project Manager is to decouple the initial instructions provided by the user into multiple commands that can be supported by other agents and executed sequentially. The presence of the Project Manager enables other agents capable of executing specific commands to receive direct and clear command requirements, eliminating the need to analyze and extract the information they require from potentially complex and abstract instructions. Consequently, this facilitates the entire system in addressing a wide range of user instructions with greater ease. Furthermore, the project manager can facilitate multiple rounds of interaction with the user, allowing for the reprocessing of vehicles previously modified in the scene, to meet the user's satisfaction requirements.

% \textbf{Project Manager Agent.} The Project Manager Agent interprets complex user requirements and breaks them down for each Technique Agent. It addresses the challenge of processing mixed and abstract user instructions by dividing them into simpler, actionable tasks for other agents. This ensures clear and direct commands, avoiding the need for agents to decipher complex instructions. The Project Manager enhances the system's ability to handle diverse instructions and enables iterative interactions with users for refining previously modified vehicles in the scene, ensuring user satisfaction.

\subsection{Specific Agent's Functionality}
\vspace{-1mm}
\quad
Agents in \textit{ChatSim} comprise two key components: a Large Language Model (LLM) and the corresponding role functions. The LLM is responsible for understanding the received commands while the role functions process the received data. Each agent is equipped with unique LLM prompts and role functions tailored to their specific duties within the system. To accomplish their tasks, agents first convert the received commands to a structured configuration using LLM with the assistance of prompts. 
% The configuration is restricted to be structured to mitigate the hallucination risk \cite{hong2023metagpt}. 
Then the role functions utilize the structured configuration as parameters to process the received data and produce the desired outcomes; see an agent example on the right side of Figure \ref{Fig:overview}. This workflow endows agents with both language interpretation capabilities and precise execution capabilities.

\noindent\textbf{Project Manager Agent.} The project manager agent decomposes direct commands into clear natural language instructions dispatched to other editing agents.
To equip the project manager agent with the capability of command decomposition, we design a series of prompts for its LLM. The core idea of the prompts is to describe the action set, give the overall goal, and define the output form with examples; 
% see the prompt detail in the appendix. 
The role functions send the decomposed instructions to other agents for editing. The presence of the project manager agent enhances the system's robustness in interpreting various inputs and streamlines operations for clarity and fine granularity.

\noindent\textbf{Tech agent for view adjustment.}
The view adjustment agent generates suitable extrinsic camera parameters. The LLM in the agent translates the natural language instructions for viewpoint adjustment into movement parameters to the target viewpoint's position and angle. In role functions, 
these movement parameters are turned into transformation matrices required by the extrinsic, which are then multiplied by the original parameters to yield a new viewpoint. 
% The resulting new extrinsics are utilized by the Background Rendering Agent and the Foreground Rendering Agent to obtain observational results from the specific viewpoint.

\noindent\textbf{Tech agent for background rendering.}
% The main task of the Background Rendering Agent is to render the relevant background for the desired scene for the end user. This agent reconstructs the scene using the user's initial input of scene photos. In this process, the agent uses NeRF to implicitly represent the entire scene, and uses our optimized NeRF technology to reconstruct high-quality multi-camera input, enabling larger-scale reconstruction and more free observation angles for rendering. Additionally, our optimized NeRF technology allows the NeRF training process to consider the shutter speed during camera capture, and directly obtains an HDRI panorama from NeRF to provide more detailed foreground object rendering to the Foreground Rendering Agent. The specific technical details will be explained in section **.
% After reconstructing the input scene, according to user needs, the Background Rendering Agent utilizes the View Adjustment Agent to provide the extrinsic rendering for observation and renders the final returned background image. The generated background frames are further passed on to the Vehicle Deleting Agent for potential deletion operations, and are then composed with the subsequent foreground rendering results to form the final output.
The background rendering agent renders the scene background based on multi-camera images. The LLM receives the rendering command and then operates the role functions for rendering. Notably, in role functions, we specifically integrate a novel neural radiance field method (McNeRF) taking multi-camera inputs and considering exposure time, solving the problem of blurring and brightness inconsistency in multi-camera rendering, see more details in Section \ref{subsec:bg_rendering}.

% It employs a novel optimized version of Neural Radiance Fields (NeRF) for large-scale scene reconstruction and flexible viewing positions and angles. This technology also incorporates shutter speed considerations during camera capture, allowing for HDRI panorama creation that aids in detailed foreground rendering. Specific technical aspects will be covered in section**. 

% The Background Rendering Agent collaborates with the View Adjustment Agent for extrinsic rendering and passes the background frames to the Vehicle Deleting Agent for possible deletions. 

\noindent\textbf{Tech agent for vehicle deleting.}
% The main task of the Vehicle Deleting Agent is to remove the vehicles that appear in the background specified by the user. The Project Manager will delegate operations involving the deletion of vehicles within the scene to the Vehicle Deleting Agent. To accomplish this, the agent first uses a scene perception model to obtain the 3D bounding boxes of any vehicles that have appeared in the scene, which are used to determine their 3D positions. These bounding boxes also serve as understanding information of the scene that can be shared with other agents. Subsequently, the Vehicle Deleting Agent calls relevant functions to obtain different attributes of the different vehicles in the scene. Using this information, the agent identifies the objects mentioned in the user's request. Finally, once the user's mentioned objects are confirmed, the agent deletes them by calling an inpainting function (such as latent diffusion methods like~\cite{rombach2021highresolution}).
The vehicle deleting agent removes specified vehicles from the background. It first identifies current vehicle attributes like 3D bounding boxes and colors from given scene information or results from a scene perception model like \cite{liu2023bevfusion}. The LLM gathers attributes of the vehicles and performs matching with user requests. Upon confirming the targeted vehicles, it employs a per-frame inpainting model as the role functions, such as latent diffusion methods~\cite{rombach2021highresolution}, to effectively delete them from the scene. 
% The images modified by the vehicle deleting agent stand for the scene backgrounds as a part of the final editing result. 

\noindent\textbf{Tech agent for 3D asset management.}
% The responsibility of the 3D Asset Management Agent is to manage a large number of 3D assets and select or modify the appropriate assets based on user needs. The Project Manager will transmit relevant information regarding added objects to the 3D Assets Management Agent. Users' requirements for adding objects may be very specific, requiring the addition of specific objects, and they may also specify detailed information about these objects, such as color, texture, etc. Based on the information in the user's input instructions, the agent determines the 3D assets needed by the user and selects them from the 3D asset bank. It also modifies relevant information about the assets according to the user's needs, and finally hands over the appropriate 3D assets to subsequent agents for final rendering of the foreground objects.
The 3D asset management agent selects and modifies 3D digital assets according to user specifications. It constructs and maintains a 3D digital asset bank; see our bank details in the Appendix. To facilitate the addition of various objects, the agent first uses LLM to select the most suitable asset by key attributes matching with the requirements, such as color and type. If the matching is not perfect, the agent could modify the asset through its role functions like changing the color.

% provides the appropriately modified asset through role functions to the Foreground Rendering Agent for foreground rendering.

\noindent\textbf{Tech agent for vehicle motion.} 
% The Vehicle Motion Agent is responsible for generating the motion of the added vehicles in the scene based on user needs. The Project Manager will convey descriptive information about the motion of added vehicles to this agent for processing. Users may provide motion information in the description of the foreground vehicles they want to add and expect to obtain the final dynamic output. This agent generates the relevant map information in the scene to assist in the subsequent motion generation. First, it generates the map information related to the scene to assist in the subsequent motion generation; then, based on the user's needs, it determines the initial placement position of the vehicle; finally, it combines the initial position and the user's needs for motion to obtain the final motion.
% The specific generation process of motion is as follows: first, using the user's input instructions, find the final destination in the map. Then, based on the starting point and destination point, fit a quadratic Bezier curve. The initial fitting result may not completely match the driving mode of the current road segment, so adjustments need to be made to the preliminary fitting result. For the adjusted trajectory, based on user instructions and map information, modify intermediate points to close Lane nodes and divide them into multiple sections. Then fit Bezier curves for each section. After multiple iterations, a motion that conforms to map information can be obtained.
The vehicle motion agent creates the initial places and subsequent motions of vehicles following the requests. Existing vehicle motion generation methods cannot directly generate motion purely from text and the scene map. To solve the problem, here we propose a novel text-to-motion method. The key idea is linking a placement and planning module as role functions with LLMs to extract and turn motion attributes into coordinates.
Motion attributes include position attributes (e.g., distance, direction) and movement attributes (e.g., speed, action). 
% Then the role functions generate the initial placement and motion given the scene lane map and the extracted attributes. 
% The scene lane map can be obtained by map estimation methods like \cite{liao2022maptr,liao2023maptrv2} if the ground-truth map is inaccessible. 
For the placement module, we endow each lane node in the lane map with its attributes to match with the position attributes. The planning module plans the vehicle's approximate destination lane node and then plans the intermediate trajectory by fitting the Bezier curves. 
% To further avoid out-of-road driving, we modify intermediate points to align with the closest lane node, dividing motion into sub-curves and fitting Bezier curves for each. 
% Through multiple iterations, a motion path that adheres to the map information is achieved. 
We also add trajectory tracking to fit vehicle dynamics; see more details in the Appendix. 


\noindent\textbf{Tech agent for foreground rendering.}
% The Foreground Rendering Agent is responsible for utilizing information input from other agents, including extrinsic, 3D assets, and their corresponding motion, to render the foreground objects in the entire scene. The rendering work is carried out by calling the relevant tools of Blender, and in order to enhance the rendering's authenticity and make the added foreground objects more consistent with background features, this agent also further calls the lighting estimation function to restore the HDRI of the entire background scene. We have optimized the lighting estimation function. Compared with traditional lighting estimation methods, our lighting estimation function can first utilize multi-camera information to fuse the lighting estimation of different cameras and restore more complete and accurate lighting information of the scene. At the same time, the lighting estimation function also uses the information contained in the Background Rendering Agent's reconstructed NeRF, which can generate background HDRI for different spatial positions and combine it with the estimated sky dome, so that the lighting information can more delicately consider the relevant background in the scene. The specific technical details will be explained in Section **.
The foreground rendering agent integrates camera extrinsic infomation, 3D assets, and motion information to render foreground objects in the scene. Notably, to seamlessly integrate the external assets with the current scene, we design a multi-camera lighting estimation method (McLight) into the role functions, coupling with McNeRF. The estimated illumination is then utilized by Blender API to generate foreground images. The detailed technical aspects will be elaborated in Section \ref{sec:fg_rendering}.

\subsection{Agent Collaboration Workflow}
\vspace{-1mm}
\quad
Agents with tailored functions collaboratively work together to edit based on user commands. The project manager orchestrates and dispatches instructions to editing agents. The editing agents form two teams: background generation and foreground generation. For background generation, the background rendering agent generates rendered images using the extrinsic parameters from the view adjustment agent, followed by inpainting by the vehicle deleting agent. For foreground generation, the foreground rendering agent renders the images using the extrinsic parameters from the view adjustment agent, selected 3D assets from 3D asset management agent, and generated motions from vehicle motion agent. Finally, the foreground and background images are composed to create and deliver a video to the user. The editing information in each agent's configuration is recorded by the project manager agent for possible multi-round editings.

\section{Novel Rendering Methods}
\vspace{-1mm}
\quad
Based on the collaborative LLM agents framework introduced in Section~\ref{sec:3}, this section presents two novel rendering techniques to enhance photo-realism in simulations. To tackle the rendering challenges caused by multiple cameras, we propose multi-camera neural radiance field (McNeRF), a novel NeRF model considering the varied camera exposure times for visual consistency. To render realistic external digital assets with location-specific lighting and accurate shadows, we propose McLight, a novel hybrid lighting estimation method combined with our McNeRF. Note that McNeRF and McLight are leveraged by the background rendering agent and the foreground rendering agent, respectively.



\subsection{McNeRF for Background Rendering} 
\label{subsec:bg_rendering}
\quad
An autonomous vehicle typically equips multiple cameras to achieve a comprehensive perception view. However, this poses challenges for NeRF training due to the misaligned multi-camera poses from asynchronized camera trigger times and the brightness inconsistency originating from different exposure times. To address these challenges, the proposed McNeRF uses two techniques: multi-camera alignment and brightness-consistent rendering.
% adopts a multi-camera alignment strategy that effectively diminishes noise in the extrinsic parameters, and exploits the exposure time of each cameras in HDR space to promote brightness consistency.

\noindent\textbf{Multi-camera alignment.} 
% Though an autonomous vehicle has a localization module to regularly obtain the precise camera poses, there is an issue with the asynchronization of camera trigger times across multiple cameras.
Autonomous vehicles, despite having a localization module for accurate camera poses, face challenges with asynchronous trigger times across multiple cameras. To align camera extrinsics for NeRF training, our core idea is to leverage a consistent spatial coordinate system provided by Agisoft Metashape~\cite{agisoft2019metashape} to align the images captured by multiple cameras at different timestamps. 

% Specifically, let $\xi^{(i,t)}$ represent the pose of the $i$th camera at the $t$th timestamp in the vehicle's global coordinate space. It is important to note that, even at the same timestamp, the shutter times of multiple cameras may differ, thereby introducing noise into $\xi^{(i,t)}$. The denoised camera pose is obtained as


Specifically, let $\mathcal{I}^{(i,k)}$ and $\mathcal{\xi}^{(i,k)}$ be the image captured by the $i$th camera at the $k$th trigger and the corresponding camera pose in the vehicle's global coordinate space, respectively. We first input all images into Metashape for recalibration.
% {\HC It is important to note that, even at the same timestamp, the shutter times of multiple cameras may differ, thereby introducing noise into $\mathcal{\xi}^{(i,t)}$.} 
The aligned camera pose is then obtained as:
% \begin{equation*}
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
%     \widehat{\xi}^{(i,k)} = T_{M \rightarrow G} \cdot f_M( \mathcal{I}^{(i,k)} ),
% \end{equation*}
\begin{equation*}
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
    \widehat{\xi}^{(i,k)} = T_{M \rightarrow G} \cdot \xi_{M}^{(i,k)},
\end{equation*}
where $\xi_{M}^{(i,k)}$ denotes the recalibrated camera pose in the Metashape's unified spatial coordinate space, and $T_{M \rightarrow G}$ is the transformation from the Metashape's coordinate space to the vehicle's global coordinate space. After alignment, the pose noise can be significantly reduced. Then, the aligned camera pose $\widehat{\xi}^{(i,t)} $ can be used to generate the origins and directions of rays for McNeRF, enabling high-fidelity rendering. The aligned pose can also facilitate the foreground rendering agent's operations.

% \begin{equation*}
% S=\frac{T^{(M)}_1 - T^{(M)}_0}{T^{(W)}_1 - T^{(W)}_0}
% \end{equation*}
% \begin{equation*}
% R_t = R^{(W)}_0 (R^{(M)}_0)^{-1} R^{(M)}_t,
% \end{equation*}
% \begin{equation*}
% T_t = \frac{R^{(W)}_0 (R^{(M)}_0)^{-1} (T^{(M)}_t - T^{(M)}_0)}{S} + T^{(W)}_0,
% \end{equation*}
% \begin{align*}
% R_{C_i, t} &= R^{(target)}_{C_0, 0} (R^{(M)}_{C_0, 0})^{-1} R^{(M)}_{C_i, t} \\
% T_{C_i, t} &= \frac{R^{(target)}_{C_0, 0} (R^{(M)}_{C_0, 0})^{-1} (T^{(M)}_{C_i, t} - T^{(M)}_{C_0, 0})}{S} + T^{(target)}_{C_0, 0}, \\
% \end{align*}

% Different from conventional NeRF, we let our radiance field's MLPs predict an HDR light intensity instead of RGB color in LDR space. This can alleviate the challenges of modeling some overexposed areas when performing within the LDR space, and facilitate the subsequent construction of the HDR environment map for foreground rendering. 
% \Note{1. what is this functionality? input, output. 2. which agent will use this functionality? 3. what is the current chllange? 4. what is our intuition to fix this issue?}

\begin{figure}[t] 
\centering
\includegraphics[width=0.47\textwidth]{imgs/rendering.pdf}
\vspace{-3mm}
\caption{\small Rendering framework. The main components include McNeRF and McLight. Background rendering uses McNeRF to predict HDR pixel value and convert it to LDR with sRGB OETF. McLight includes a skydome lighting estimation network and adopts McNeRF to generate surrounding lighting.}
\label{fig:rendering_pipeline}
\vspace{-6mm}
\end{figure}

\noindent\textbf{Brightness-consistent rendering.} 
The exposure times of cameras can differ substantially, causing significant brightness differences across images, hindering the NeRF training. As shown in Figure~\ref{fig:rendering_pipeline}, McNeRF, addresses this by incorporating exposure times into HDR radiance fields, prompting brightness consistency.

% To render the color of each pixel, we cast the ray  $\mathbf{r}$ from the camera center $\mathbf{o}$ with direction $\mathbf{d}$. 
%We sample a sequence of $K$ points from this ray; that is, $\mathbf{r}_k = \mathbf{o} + \ell_k \cdot \mathbf{d}$, where $\ell_k$ is a length. For each sampled point $\mathbf{r}_k$, \
We adopt F2-NeRF~\cite{wang2023f2} as our backbone model to handle the unbounded scene, sampling $K$ points along the ray $\mathbf{r}$ and estimating each point's HDR radiance $\mathbf{e}_k$ and density $\sigma_k$. The HDR light intensity is then calculated as:
\begin{equation}
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
    \widehat{\mathcal{I}}_{\rm HDR}(\mathbf{r}) = f(\Delta t) \cdot  \sum^K_{k=1} T_k \alpha_k \mathbf{e}_k,
\label{eq:nerf}
\end{equation}
where $\alpha_k = 1-\text{exp}(-\sigma_k \delta_i)$ is the opacity, $\delta_i$ is the point sampling interval, $T_k = \prod^{k-1}_{i=0} (1-\alpha_i)$ is the accumulated transmittance and $\Delta t$ is the exposure time. The normalization function $f(\Delta t) = 1 + \epsilon (\Delta t - \mu)/{\sigma}$ is designed to stabilize training, where $\epsilon$ is a hyperparameter for scaling, $\mu$ and $\sigma$ are the mean and standard deviation of the exposure times of all images, respectively.

% By integrating exposure time into the rendering process, McNeRF recovers scene radiance in HDR linear space\Note{zi: in a way that obeys the laws of physics} to tackle the pixel color inconsistency at two camera images with different exposure times.
By predicting scene radiance in HDR and multiplying it by the exposure time, we recover the light intensity received by the sensor and tackle the inconsistent color supervision at the intersections of two camera images with distinct exposure times.
% and further achieves more consistent brightness when rendering ultra-wide angle images. 
Moreover, the HDR light intensity outputted by McNeRF can provide scene-level illumination for foreground object rendering, a topic further discussed in Section~\ref{sec:fg_rendering}. %\Note{sc: any other reason to use HDR?}

% Our rendering method presents two significant advancements compared to standard NeRFs. First, integrating the exposure time into the rendering process enables the network to dynamically adjust the lighting conditions in accordance with the varying exposure times of individual cameras. Here the specific increasing function $f(\cdot)$ is intentionally designed to stabilize the network’s training, enhancing the model's adaptability to diverse lighting scenarios. Second, different from the common practice of using the LDR light intensity, our method outputs the HDR light intensity. This shift to HDR aligns more closely with the illumination estimation, which will be further discussed in Section~\ref{sec:fg_rendering}.

To train the rendering network, we enforce the consistency of radiance between the rendered image (prediction) and the captured image (ground-truth). Given the ground-truth image $\mathcal{I}$, the loss function is then:
\begin{equation*}
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\mathcal{L} = \frac{1}{|R|} \sum_{\mathbf{r} \in R} \left(\mathrm{OETF}\left(\widehat{\mathcal{I}}_{\rm HDR}(\mathbf{r}) \right) - \mathcal{I}(\mathbf{r}) \right)^2,
\end{equation*}
where $R$ represents the ray set and $\mathrm{OETF}(\cdot)$ is the sRGB opto-electronic transfer function (gamma correction)~\cite{international1999iec} that converts HDR light intensity to LDR colors.


% \subsubsection{Agents of Editing Tech}

% This section includes several executors capable of fulfilling the user's editing requirements for the scene. It receives more specific sub-tasks assigned by the agent of project manager and, with the aid of rendering, lighting conditions, and other tools provided by the agent of supporting tech, completes operations such as viewpoint transformation, vehicle deletion, trajectory generation, and rendering. We will discuss the specific functions of each agent in detail below.

\subsection{McLight for Foreground Rendering} 
\label{sec:fg_rendering}
% To enrich the content of the scene with a substantial amount of digital 3D assets, we employ a traditional graphics pipeline (like Blender) for rendering 3D models. To seamlessly incorporate the rendered 3D assets into the background image without any sense of discordance, we need to accurately reproduce the lighting of the scene. 

% \subsubsection{Hybrid Spatial-Varying Lighting Estimation}
% We propose a novel spatial-varying hybrid lighting estimation from multi-view images, where the skydome and the scene illumination are modeled separately. The skydome is considered as invariant, while the illumination originating from the scene varies with the given location. The autonomous driving scenes typically consist of complex geometric structures like buildings or trees, which results in location-specific lighting effects such as shadows and reflections. We first elaborate how to estimate the sky dome and recover scene lighting from our Radiance Field.
\quad
To enrich the scene's content with substantial digital 3D assets, we employ Blender~\cite{blender} foreground virtual objects' rendering. A seamless insertion critically depends on accurately estimating the scene's illumination conditions. Thus, as shown in Figure~\ref{fig:rendering_pipeline}, we propose McLight, a novel hybrid lighting estimation consisting of skydome lighting and surrounding lighting.
% \Note{sc: you only describe the procedure; need to show technical novelty of McLight}



\noindent\textbf{Skydome lighting estimation.}
% Restoring skydome lighting from single or multiple images is challenging due to the absence of corresponding HDR ground truth. To solve this dilemma, we first utilize external HDR data to train an HDR skydome reconstruction network, which represents skydome characteristics into latent vectors. Then, we can use multi-camera images to estimate the latent vector effectively and restore skydome lighting.
% \Note{sc: you only describe two steps; need to highlight technical novelty of Skydome lighting estimation}
% Restoring skydome lighting from images is challenging due to the absence of corresponding HDR ground truth. We design a two stages approach to solve this. We train a specialized HDR skydome reconstruction network with self-collected external HDR data in the first stage. This network features an innovative residual connection bridging latent vectors and HDR output, effectively addressing the issue of the decoder network output being too smooth. In the second stage, we develop a self-attention for fusing multi-camera latent vectors to exploit complementary visual cues.
Estimating skydome lighting from images is challenging for restoring accurate sun behavior. To achieve this, we propose a novel residual connection from the estimated peak intensity to the HDR reconstruction to address over-smoothing output. Further, we adopt a self-attention mechanism to fuse multi-camera inputs, capturing complementary visual cues. 
% Here is our two-stage training process.
% \Note{sc: residual connection and self-attention fusion module are quite detailed. what is the issue in Restoring skydome lighting? } \Note{zi: This network incorporates two innovative designs: a residual connection bridging latent vectors and HDR output, and a self-attention fusion module. These advancements address the issue of insufficient peak sunlight value estimation encountered in previous works.}
% Following [], we encode the LDR skydome to 3 intermediate vector $\mathbf{f}_{dir} \in \mathbb{R}^{3}, \mathbf{f}_{int} \in \mathbb{R}^{3}_{+}$ and $\mathbf{f}_{latent} \in \mathbb{R}^{64}$. $\mathbf{f}_{dir}$ represents the peak direction, $\mathbf{f}_{int}$ represents the peak intensity and $\mathbf{f}_{latent}$ controls the content and the color of the sky. We then use a decoder network to reconstruct the HDR sky. We observed that using $\mathbf{f}_{int}$ as an input to a decoder network in [] was insufficient for restoring high brightness levels in the reconstructed HDR image.  We train the sky reconstruction network on a set of outdoor HDR panoramic images collected by us and kept the decoder fixed. By estimating the intermediate vectors from multi-view images, we are able to utilize the trained decoder to reconstruct the illumination map of the sky.
% Current skydome estimation methods exhibit two notable shortcomings. First, these methods predominantly use LDR colors to depict the skydome. However, the limited LDR range fails to adequately capture the full intensity of the sun's brightness, causing a less accurate representation. Second, the prevalent sky dome estimation techniques are tailored for single-camera setups. Consequently, they lack compatibility with systems that incorporate inputs from multiple cameras. To address these two issues, our multi-view sky dome estimation adopts a two-stage training: HDR-based single-camera skydome estimation and multi-camera fusion.


Here we employ a two-stage process. In the first stage, we train an autoencoder to reconstruct the corresponding HDR panorama from an LDR panorama. Following ~\cite{wang2022neural}, the encoder transforms the LDR skydome panorama into three intermediate vectors, including the peak direction vector $\mathbf{f}_{\rm dir} \in \mathbb{R}^{3}$, the intensity vector $\mathbf{f}_{\rm int} \in \mathbb{R}^{3}_{+}$, and the sky content vector $\mathbf{f}_{\rm content} \in \mathbb{R}^{64}$. However, as HDR intensity behaves like an impulse response at its peak position, with pixel values thousands of times higher than its neighbors,  it is difficult for the decoder to recover such patterns. To tackle this, we design a residual connection that injects $\mathbf{f}_{\rm int}$ into the decoded HDR panorama with a spherical Gaussian lobe attenuation. This explicitly restores the peak intensity of the sun in the reconstructed HDR panorama, allowing us to render strong shadows for virtual objects. 

% Noticing the inadequacy of using $\mathbf{f}_{int}$ as an input to a decoder network $\mathbf{f}_{int}$ for restoring high brightness levels in the reconstructed HDR image, we innovate by introducing a residual connection that directly infuses $\mathbf{f}_{int}$ into the HDR reconstruction.  We use a spherical Gaussian lobe to simulate the luminance attenuation around the peak direction, explicitly restoring the sun's illumination. The trained decoder then will be fixed and utilized for the subsequent process of estimating environmental lighting from autonomous driving images input.

In the second stage, we train an image encoder and a multi-camera fusion module built upon the pretrained decoder from the first stage. Specifically, for images from each camera, a shared image encoder predicts the peak direction vector $\mathbf{f}_{\rm dir}^{(i)}$, the intensity vector $\mathbf{f}_{\rm int}^{(i)}$, and the sky content vector $\mathbf{f}_{\rm content}^{(i)}$ for each image $\mathcal{I}^{(i)}$, where $i$ is the camera index. We design the latent vector fusion across the multiple camera views as follows: all $\mathbf{f}_{\rm dir}^{(i)}$ are aligned to the front-facing view using their extrinsic parameters and averaged to form $\bar{\mathbf{f}}_{\rm dir}$; all $\mathbf{f}_{\rm int}^{(i)}$ are averaged to yield $\bar{\mathbf{f}}_{\rm int}$; all $\mathbf{f}_{\rm content}^{(i)}$ are integrated into $\bar{\mathbf{f}}_{\rm content}$ through a self-attention module. Finally, the pretrained decoder reconstructs the HDR skydome image $\mathcal{I}_{\rm skydome}$ from $\bar{\mathbf{f}}_{\rm dir}$, $\bar{\mathbf{f}}_{\rm int}$ and $\bar{\mathbf{f}}_{\rm content}$. 
% Here the decoder is freezed and the encoder and fusion operations are trainable.

Compared to alternative approaches~\cite{wang2022neural,hold2019deep}, our multi-camera sky dome estimation technique accurately reproduces the sun's intensity response behavior at its peak with our residual designs, significantly improving the accuracy and fidelity of the skydome reconstruction. %\Note{sc: why it can achieve this? }

\begin{figure}[t] 
\centering
\includegraphics[width=0.42\textwidth]{imgs/mix_result_3frame.png}
\vspace{-3mm}
\caption{\small Editing result under a complex and mixed command.}
\label{fig:mix_result}
\vspace{-5mm}
\end{figure}


\noindent\textbf{Surrounding lighting estimation.}
Merely modeling the skydome cannot replicate the complex location-specific lighting effects, like those in the shade with sunlight blocked by trees or buildings. 
% Thus, it is crucial to consider and recover the surrounding scene's influence on lighting. 
Our McNeRF is capable of storing precise 3D scene information, enabling us to capture the surrounding scene's impact on lighting. This approach facilitates the achievement of spatially-varying lighting estimation. Specifically, we sample the hemisphere rays at the virtual object's position $\textbf{o}$.
The rays' directions, $\textbf{d}_i, i=0, 1, \cdots, h\times w$, are aligned with pixel coordinates on a unit sphere using equirectangular projection from an environment map, where $h$ and $w$ are map's height and width. With the ray $\mathbf{r} = \mathbf{o} + t\mathbf{d}_i$, we query our McNeRF as Equation~\ref{eq:nerf} to obtain HDR surrounding lighting $\mathcal{I}_{\rm surround} (\textbf{o}, \textbf{d}_i)$. The surrounding lighting estimation reconstructs complex environmental lighting, achieving a spatially varying effect and high consistency with the background.
 % \Note{sc: highlight technical novelty of Surrounding lighting estimation}
% The directions of these rays $\textbf{d}_i, i=0, 1, ..., N$ corresponds with the coordinates of pixels from the environment map projected onto a unit spherical surface with equirectangular projection, where $N$ is the pixel number of the environment map. 
% \begin{equation*}
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% \mathcal{I}_{\rm surround} (\textbf{o}, \textbf{d}_i) = f(\Delta t)\sum^K_{k=1} T_k \alpha_k \mathbf{e}_k, 
% \end{equation*}
% where $f(\Delta t)$, $T_k$ and $\alpha_k$ are computed as Sec~\ref{subsec:bg_rendering}. 

 % {\HC Since McNeRF is already trained in background rendering pass, we only need to query the ray here, leading to high consistency with the background while reducing model complexity.}  \Note{sc: put this earlier. } 



\noindent\textbf{Blending.}
% After passing through the final sampling point, the light ray can retain a certain level of transmittance. We consider that this final portion will fully receive the illumination from the skydome. 
We blend the HDR intensity value from the skydome and surrounding lighting by transmittance of the final sampling point from McNeRF. The idea is that the rays emitted outside the radiance fields will definitely hit the skydome. Given the direction $\textbf{d}_i$, we retrieve the skydome's intensity $\mathcal{I}_{\rm skydome}(\textbf{d}_i)$ with equirectangular projection. The final HDR light intensity $\mathcal{I}_{\rm env} (\textbf{o}, \textbf{d}_i)$ is a combination of scene and skydome: 
\begin{equation*}
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\mathcal{I}_{\rm env}(\textbf{o}, \textbf{d}_i) = \mathcal{I}_{\rm surround} (\textbf{o}, \textbf{d}_i) + T_K \mathcal{I}_{\rm skydome} (\textbf{d}_i), 
\end{equation*}
where $T_K$ is the last sampling point's transmittance. 

McLight offers two main advantages: i) it explicitly recovers the illuminance behavior at the peak and use complementary information from multiple cameras to restore accurate skydome; and ii) it enables location-specific lighting with consideration of complex scene structures.

% \subsubsection{Render Inserted Objects with Blender}
% After obtaining the precise position to be added a car and its corresponding spatially-varying illumination estimation, The agent for adding vehicles can use the rendering tools (Blender) provided by the agent of supporting tech to add vehicles in the scene.


% The Agent receives descriptions from users about the vehicles they want to add to the scene, converts these descriptions into specific RGB colors and vehicle types, and then feeds these along with the output vehicle positions from the previous agent into Blender. Blender can then render the vehicles from the asset bank into the image, taking into account spatially-varying illumination estimation. 

% The autonomous driving scenes typically consist of complex geometric structures like buildings or trees, which results in location-specific lighting effects such as shadows and reflections. These effects are too complex to be expressed merely by an environmental map. 

% \todo{Add a figure that can illustrate the effectiveness of spatially-varying illumination.(Yifan Lu, Zi Wang)}


% \subsection{Vehicle Motion} 

% Input: user's commands describing how they want the added vehicle to move

% Tools: map provided by agent of supporting tech

% Output: trajectories

% \todo{Write more details here (Chenxin Xu)}

% \subsection{3D Asset Management} 
% We collect and maintain a high-quality collection of 3D assets, which have been normalized to a standard format. This allows the GPT model to have the capability to modify various attributes of the 3D assets, such as color. Here is how we implement this...

% \subsection{View Adjustment} 
% \todo{No technical Implementation and Contribution. Shall we remove this section?}


% \subsection{Vehicle Deleting} 
% \todo{No technical Implementation and Contribution. Shall we remove this section?}







% \textbf{Agent for output generation}


% \begin{figure*}[htbp]
% \centering
% \begin{minipage}[t]{0.49\textwidth}
% \centering
% \includegraphics[width=0.97\textwidth]{imgs/mix_result.png}
% \caption{Example of generation result under a complex and mixed prompt.}
% \end{minipage}
% \begin{minipage}[t]{0.49\textwidth}
% \centering
% \includegraphics[width=0.97\textwidth]{imgs/semantic_result.png}
% \caption{Example of generation result under a highly semantic prompt.}
% \end{minipage}
% \end{figure*}

% \begin{figure}[t] 
% \centering
% \includegraphics[width=0.42\textwidth]{imgs/mix_result_3frame.png}
% \vspace{-3mm}
% \caption{\small Editing result under a complex and mixed command.}
% \label{fig:mix_result}
% \vspace{-5mm}
% \end{figure}

\begin{figure}[t] 
\centering
\includegraphics[width=0.42\textwidth]{imgs/semantic_result_3frame.png}
\vspace{-3mm}
\caption{\small Editing result under a highly abstract command.}
\label{fig:abstract_result}
\vspace{-4mm}
\end{figure}

==> sec/4_experiments.tex <==
\section{Experimental Results}
\subsection{Datasets and implementation details}
\vspace{-1mm}
\quad
We demonstrate a variety of results mainly on the Waymo Open Dataset~\cite{Sun_2020_CVPR}, which contains high-quality multi-camera images and the corresponding calibrations. For McLight skydome estimation, we collect 449 HDRIs from online HDRI databases for the autoencoder training and use HoliCity \cite{zhou2020holicity}, a street view panorama dataset for the second stage; see more dataset details in the Appendix.

In our experiment, we use front, left front, and right front cameras in each frame. During the rendering process, we choose 40 frames per scene at a 10Hz sampling rate, totaling 120 images. We evenly select $1 / 8$ of these as the test set, with the remainder used for training. The input images are used at the dataset's initial resolution of $1920 \times 1280$; we employ GPT-4 as the LLMs in all of our experiments; see more implementation details in the Appendix.
% reconstructing and rendering * selected scenes. Each scene employed data from three cameras: Front, Front Left, and Front Right, for training. Throughout the training of all scenes, the inputs from these three distinct cameras shared all the Neural Radiance Field (NeRF) parameters. During the rendering process, we chose 40 frames per scene (at a 10Hz sampling rate), amounting to a total of 120 images for training. The input images were used at the dataset's initial resolution of 1920x1280.

\subsection{System results}
\label{subsec:system_results}
\textbf{Editing via language commands.} We select three representative commands to demonstrate the editing results. All of the results demonstrate we achieve photo-realistic wide angle results, thanks to McNeRF and McLight.

\emph{Mixed and complex command.} We send the system with a mixed and complex command, implying that a police car is chasing a wrong-way racer. The target scene, command and the result are shown in Figure \ref{fig:mix_result}. We see that i) every requirement in the complex command is accurately executed thanks to our multi-agent collaboration design; ii) this command successfully simulates one rare but dangerous driving condition, which is significant in accident testing. 

\emph{Highly abstract command.} The second type is a highly abstract command. The inputs and results are presented in Figure \ref{fig:abstract_result}. We see that i) this highly abstract command is hard to decompose by sentence division but still can be correctly executed by our method, and ii) our 3D asset bank offers a large variety of objects for addition.

% \begin{figure}[t] 
% \centering
% \includegraphics[width=0.42\textwidth]{imgs/semantic_result_3frame.png}
% \vspace{-3mm}
% \caption{\small Editing result under a highly semantic command.}
% \label{fig:semantic_result}
% \vspace{-4mm}
% \end{figure}


% \begin{figure*}[t] 
% \centering
% \includegraphics[width=0.97\textwidth]{imgs/interactive_result.png}
% \vspace{-4mm}
% \caption{\small Generation under multi-round interactive prompts.}
% \label{fig:interactive_result}
% \vspace{-5mm}
% \end{figure*}

\begin{figure}[t] 
\centering
\includegraphics[width=0.47\textwidth]{imgs/interactive_result_2round_1.png}
\vspace{-3mm}
\caption{\small Editing result under multi-round commands.}
\label{fig:interactive_result}
\vspace{-5mm}
\end{figure}



\emph{Multi-round command.} We also perform a multi-round chat with our system, and the commands in different rounds exist context dependencies. The final results are shown in Figure \ref{fig:interactive_result}. We see that i) our system is well-equipped to handle multi-round commands and execute the commands in each round precisely; ii) our system can handle the context dependencies across different rounds 
thanks to the recording ability of the project manager agent.
% the multi-round interaction ability enables ChatSim to finetune and iterate the user's commands in a full interaction process.


\begin{figure}[t] 
\centering
\includegraphics[width=0.45\textwidth]{imgs/comparison_system.png}
\vspace{-3mm}
\caption{\small Qualitative comparison with Visual Programming\cite{gupta2023visual}. }
\label{fig:comparison_system_result}
\vspace{-4mm}
\end{figure}
\noindent\textbf{Comparison with Visual Programming~\cite{gupta2023visual}.}
Visual Programming (VP) is the latest SoTA language-driven 2D image neuro-symbolic system, which can also be used for editing with language commands. Given that Visual programming only supports editing of single frames in 2D images, we limit our comparison to the deletion and replacement operations within the original view that it can support. The comparison in Figure \ref{fig:comparison_system_result} shows that \textit{ChatSim} significantly outperforms VP in the two samples. Actually, in our extensive experiments, VP fails in most cases. The reason is that VP only has a single agent, making it difficult to handle mixed tasks. In comparison, \textit{ChatSim} has multiple collaborative agents with specific roles, ensuring accurate task execution.
% can split and execute specific tasks through multi-agent collaboration.

%, based on a multi-agent division of labor approach, analyzes and decomposes instructions into executable commands. It operates based on the 3D information of the scene to complete editing operations on the 3D scene. Such editing methods cannot be properly accomplished by Visual programming, which relies on 2D image-based editing techniques.

% even for 2D image editing, Visual Programming struggles to perform scene editing operations in almost all scenarios; and ii) ChatSim can leverage its comprehensive multi-agent collaboration framework to accurately analyze and execute requirements, ultimately delivering results that meet user needs.


% \begin{table}[t]
% \scriptsize
% \centering
% \setlength\tabcolsep{12pt}
% \resizebox{.9\columnwidth}{!}{
% \begin{tabular}{c|ccc}
% \toprule
%    Data source                & AP30 & AP50 & AP70  \\
% \hline
%  % Real &   BevFormer        &                  &   \\    
%  % Real+Sim &   BevFormer        &                  &   \\ 
%  Real        & 0.352 & 0.214 & 0.043   \\    
%  Real+Sim    & \textbf{0.364} & \textbf{0.222} & \textbf{0.062}   \\ 
% \bottomrule
% \end{tabular}}
% \vspace{-3mm}
% \caption{\small Comparison of detection model performance w/o and w/ our simulated data.}
% \label{tab:augmentation_exp}
% \vspace{-6mm}
% \end{table}

\begin{figure}[t] 
\centering
\includegraphics[width=0.46\textwidth]{imgs/data_augment_comparison.png}
\vspace{-3mm}
\caption{\small Comparison of detection performance w/o and with our simulated data under different amounts of real data during training. }
\label{fig:data_augment_comparison}
\vspace{-5mm}
\end{figure}


\noindent\textbf{3D detection with simulation data.} 
We validate the benefits of our simulation as data augmentation for a
downstream 3D object detection task on Waymo Open Dataset~\cite{sun2020scalability}. We simulate 1960 frames, derived from scenes in the training dataset. In the simulation, cars with various types, locations, and orientations are incorporated. The detection model adopts Lift-Splat~\cite{philion2020lift}. Figure \ref{fig:data_augment_comparison} shows detection performances with and without fixed augmentation under various amounts of real data. We see that i) a significant and consistent improvement across different data sizes is achieved; ii) when real data is limited, our simulation notably aids in rough detection (AP30); iii) when the amount of real data increases, our simulation further significantly improves fine-grained detection (AP70), reflecting the high-quality of our simulation.

\subsection{Component results}
\vspace{-1mm}
\noindent\textbf{Multi-agent collaboration.}
We evaluated the effectiveness of the multi-agent collaboration by checking whether the command is successfully executed in Table \ref{tab:collaboration_exp}. In scenarios without multi-agent collaboration, all operations are executed by a single LLM agent. We see that a single LLM agent leads to notably lower execution accuracy across all categories due to process limitations. In contrast, the collaborative multi-agent approach can manage most commands, attributed to its task division and agent role specificity.
% This outcome emphasizes the importance of multi-agent collaboration in handling complex tasks. By distributing the workload among specialized agents, each adept at handling specific aspects of a command, the overall system becomes more efficient and accurate in executing diverse and complex operations. This distributed approach allows for more nuanced processing of commands and significantly improves the fidelity and precision of the executed tasks.

\begin{table}[t]
\scriptsize
\centering
\setlength\tabcolsep{4pt}
\resizebox{.93\columnwidth}{!}{
\begin{tabular}{c|ccccc}
\toprule
\multirow{2}*{\makecell{Multi-agent\\collaboration}}   &\multicolumn{5}{c}{Language command category}    \\
\cline{2-6}
~& {Deletion} &  {Addition} & {View change} & {Revision} & {Abstract} \\
\midrule
 &  0.617 & 0.383 & 0.717 & 0.367 & 0.216                                  \\
\checkmark    &  \textbf{0.983} &  \textbf{0.867} & \textbf{0.967} & \textbf{0.917} & \textbf{0.883}         \\
\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{\small The accuracy (\%) of task completion by LLM without and with multi-agent collaboration. }
\label{tab:collaboration_exp}
\vspace{-4mm}
\end{table}

\begin{table}[t]
\centering
\footnotesize
\resizebox{.93\columnwidth}{!}{
\begin{tabular}{c|cccc}
\toprule
Methods   & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  & Inf. time (s)$\downarrow$ \\
\midrule
DVGO~\cite{sun2022direct}           &    23.57	&0.770	&0.508 & 7.7\\
Mip-NeRF360~\cite{barron2022mip}       &  24.40&	0.754&	0.528 & 101.8 \\
S-NeRF~\cite{xie2023s}           &    24.71  &   0.759   & 0.519 &   114.5   \\
F2NeRF~\cite{wang2023f2}          &     23.26	& 0.773&	0.439 & 2.4 \\
\midrule
Ours w/o alignment & 23.32 & 0.776 & 0.437 & 2.5\\
Ours w/o exposure & 25.18 & 0.819 & 0.381 & 2.4\\
\textbf{McNeRF (Ours)}  &   \textbf{25.82}	& \textbf{0.822} &	\textbf{0.378} &  2.5\\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\caption{\small Background novel view rendering performance evaluation. }
\label{render_exp}
\vspace{-3mm}
\end{table}
\noindent\textbf{Background rendering.}
We compare our McNeRF with several other state-of-the-art methods on the background novel view synthesis task. We perform reconstruction and rendering on 32 selected scenes. Table~\ref{render_exp} shows the quantitative results comparison on three metrics: PSNR, SSIM, and LPIPS. We see that i) McNeRF achieves SoTA performance on all three metrics, significantly outperforming other baselines; ii) McNeRF has a fast inference speed, enabling quick responses to user requests for image rendering. 
\begin{figure}[t] 
\centering 
\includegraphics[width=0.42\textwidth]{imgs/nerf_comparison_bold.png} 
\vspace{-3mm}
\caption{\small Comparisons of wide-angle images generation. (a) S-NeRF.(b) F2NeRF. (c) McNeRF (Ours). Last row: target images.}
\vspace{-4mm}
\label{Fig:nerf_comparision} 
\end{figure}

Figure~\ref{Fig:nerf_comparision} demonstrates qualitative comparisons between other methods and ours. We see that existing NeRF methods do not consider the exposure time, leading to noticeable changes in brightness at the junctions of different cameras in the image, as well as an overall inconsistency in exposure across the wide-angle view. Our method can make the brightness of the entire image more consistent.


% \begin{table}[h]
% \scriptsize
% \centering
% \begin{tabular}{c|cccc}
% \toprule
% Methods   & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  & Inf. time $\downarrow$ \\
% \midrule
% DVGO~\cite{sun2022direct}           &    23.57	&0.770	&0.508 & 7.6751\\
% Mip-NeRF360~\cite{barron2022mip}       &  24.40&	0.754&	0.528 & 101.7955 \\
% S-NeRF~\cite{xie2023s}           &    24.71  &   0.759   & 0.519 &   114.4800   \\
% F2NeRF~\cite{wang2023f2}          &     23.26	& 0.773&	0.439 & 2.3866 \\
% \midrule
% Ours w/o adjustment & 23.32 & 0.776 & 0.437 & -\\
% Ours w/o exposure & 25.18 & 0.819 & 0.381 & -\\
% Ours  &   \textbf{25.82}	& \textbf{0.822} &	\textbf{0.378} &  2.5437\\
% \bottomrule
% \end{tabular}
% \caption{Background rendering evaluation}
% \label{render_exp}
% \end{table}





\begin{table}[t]
\scriptsize
\setlength\tabcolsep{4pt}
\resizebox{.98\columnwidth}{!}{
\begin{tabular}{c|cc|cc|c}
\toprule
\multirow{2}*{Method} & \multicolumn{2}{c|}{Peak Intensity(log10) Error}  &\multicolumn{2}{c|}{Peak Angular Error (deg)} & \multirow{2}*{User study(\%) $\uparrow$}\\
~& Mean $\downarrow$  & Median $\downarrow$ & Mean $\downarrow$  & Median $\downarrow$ & ~\\
\midrule
Hold-Geoffroy et al. \cite{hold2019deep}                   & 0.899          & 0.975  & 48.4 & 51.6    &19.5     \\
Wang et al.  \cite{wang2022neural}                        & 0.590          & 0.628   &33.5&29.4    &37.3    \\
\textbf{McLight (Ours)}                           & \textbf{0.449} & \textbf{0.270} & \textbf{32.3} & \textbf{26.5} &\textbf{43.1}  \\ 
\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{\small Comparison with previous methods on lighting estimation.}
\label{tab:peak_int}
\vspace{-3mm}
\end{table}


\begin{figure}[t]
    \centering
\includegraphics[width=0.47\textwidth]{imgs/vis_compare.jpg}
    \vspace{-3mm}
    \caption{\small Comparison with different lighting estimation methods. 
    % (a) Hold-Geoffroy~\cite{hold2019deep}. (b) Wang ~\cite{wang2022neural}. (c) McLight (Ours). (d) The spatial varying effect from McLight.  
    }
    \label{fig:vis_compare}
    \vspace{-3mm}
\end{figure}


\noindent\textbf{Foreground rendering.}
We compare our McLight with the other two SoTA methods~\cite{wang2022neural,hold2019deep}. Table \ref{tab:peak_int} shows the comparison of relative intensity(log 10) error on our HDRI dataset, angular error on HoliCity~\cite{zhou2020holicity}, and user study. We see that McLight achieves more accurate peak behavior and receives noticeably higher user preferences. Figure \ref{fig:vis_compare} shows the visualizations of vehicle insertion. The vehicles added through McLight feature significantly more realistic reflections and strong shadows consistent with the scene.
% , blending seamlessly with the scene; ii) the shadows of objects introduced by McLight are more pronounced and align more consistently with the shadows of existing objects in the scene.


\begin{table}[t]
\scriptsize
\centering
\resizebox{.98\columnwidth}{!}{
\begin{tabular}{c|ccccc}
\toprule
     Methods                     & Straight & Left Turn & Right Turn & Speed & Within-road \\
\hline
 GPT2Code  &  0.738   &   0.559   &   0.536   &   0.893  &  0.214  \\
 GPT2Motion&  0.595   &   0.119   &   0.167   &   0.345  &  0.277  \\
   \textbf{Ours}    & \textbf{0.988}   &   \textbf{0.940}   &  \textbf{0.976}   &   \textbf{0.952}  &  \textbf{1.000}  \\

\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{\small Comparison with motion generation from text methods.}
\label{tab:motion_exp}
\vspace{-6mm}
\end{table}

\noindent\textbf{Vehicle motion.}
As shown in Table \ref{tab:motion_exp}, we compare the motion generation method from user commands with two of our designed baselines:  1. GPT2Motion, which directly uses LLM to return the motion coordinates; 2. GPT2Code, which first generates code using LLM and executes it to obtain the vehicle motion. We validate multiple actions in multiple scenarios and report the user study result. The user study is to determine if the generated motions matched the command intents and fitted with the lane map. We see that our method demonstrated a significant advantage in generating motions from language commands. Additionally, it maintained a high rate of keeping the trajectories within the lane boundaries. 
% Our motion generation design returns accurate and compliant results which can not be easily completed with direct methods.



% \subsubsection{Evaluation of rendered scene }
% 1. PSNR, SSIM for background: reconstruct the scene, but mask the moving vehicle. Calculate the metrics. 

% 2. Perception Evaluation and Training: Model: BEVFormer, 2D and 3D detection
% real2sim





% \begin{table}[h]
% \small
% \centering
% \begin{tabular}{cc|ccc}
% \toprule
% Methods     & Alignment methods           & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
% \midrule
% S-NeRF             &       &    24.71  &   0.76   & 0.51      \\
% Mip-NeRF360     &    /      &  24.40&	0.75&	0.53 \\
% Mip-NeRF360 &      &    25.47&	0.77&	0.51\\
% DVGO          &      /      &    23.57	&0.77	&0.51 \\
% DVGO       &      &   24.65 & 	0.79&	0.49 \\
% F2NeRF        &     /       &     23.26	& 0.77&	0.44 \\
% F2NeRF  &    &   25.18	& 0.82 &	0.38\\
% F2NeRF+exposure  &    &   \textbf{25.82}	& \textbf{0.82} &	\textbf{0.37}\\
% \bottomrule
% \end{tabular}
% \caption{Background rendering evaluation}
% \end{table}
 

% \begin{table}[t]
% \begin{tabular}{c|cc}
% \toprule
% Peak Intensity Error (log10) & Mean $\downarrow$  & Median $\downarrow$ \\ \midrule
% Hold Geoffroy                   & 0.899          & 0.975           \\
% Wang                            & 0.590          & 0.628           \\
% Ours                            & \textbf{0.449} & \textbf{0.270}  \\ 
% \bottomrule
% \end{tabular}
% \caption{Peak intensity error in our collected HDRI dataset.}
% \label{tab:peak_int}
% \end{table}

% \begin{table}[]
% \begin{tabular}{l|cc}
% \hline
% Peak Direction Angular Error & \textbf{Mean} $\downarrow$ & \textbf{Median} $\downarrow$ \\ \hline
% Hold Geoffroy                & 48.4          & 51.6            \\
% Wang                         & 33.5          & 29.4            \\
% Ours                         & \textbf{32.3} & \textbf{26.5}   \\ \hline
% \end{tabular}
% \caption{Peak angular error in Holicity dataset in degree.}
% \label{tab:peak_dir}
% \end{table}

% \begin{table}[]
% \begin{tabular}{l|c}
% \hline
% User Study    & \textbf{Percentage} \\ \hline
% Hold Geoffroy & 19.5                \\
% Wang          & 37.3                \\
% Ours          & \textbf{43.1}       \\ \hline
% \end{tabular}
% \caption{User study. Choose the most realistic from 3 image}
% \label{tab:user_study}
% \end{table}




% \begin{figure}[t] 
% \centering 
% \includegraphics[width=0.47\textwidth]{imgs/spatial_varying_wo_hdr.jpg} 
% \caption{Spatial-varying lighting effect.}
% \label{Fig:spatial_varying_light} 
% \end{figure}

% 1. FID w/wo lighting estimation
% 2. User study
% 3. Add some cars (say, 100) in the scenerios and evaluate the detection bbox confidence.
% 4. Visualization (optimal)

% \begin{figure}[!h] 
% \centering 
% \includegraphics[width=0.48\textwidth,height=0.27\textwidth]{imgs/added_cars.pdf} 
% \caption{Visualization of added cars.}
% \label{Fig:cars} 
% \end{figure}


% \begin{table}[h]
% \scriptsize
% \centering
% \begin{tabular}{c|ccc}
% \toprule
%        Illumination estimation                    & FID & User Study & Detection Confidence \\
% \hline
%  &           &                  &                           \\
% \checkmark    &           &                  & \\
% \bottomrule
% \end{tabular}
% \caption{Car adding evaluation (need to revised)}
% \end{table}

% \subsubsection{Car removal evaluation}
% 1. FID
% 2. Visualization




% \begin{figure}[!h] 
% \centering 
% \includegraphics[width=0.48\textwidth,height=0.27\textwidth]{imgs/motion.pdf} 
% \caption{Visualization of generated motions.}
% \label{Fig:motion} 
% \end{figure}

==> sec/X_supple.tex <==
% \clearpage
% \setcounter{page}{1}
% \maketitlesupplementary



\section{LLM-Agents Details}
\subsection{Agent Implement Details}
LLM-Agents consist of their LLM (Large Language Model) component and corresponding functionalities. All experiments utilize the GPT-4 API\cite{llm_gpt4} to implement the LLM part. In each agent's prompt, there are elements involving the agent's function, the definition of actions that the agent needs to perform, the definition of information inputted to the agent, and the definition of outputs required from the agent. To facilitate the integration of Python code and ensure stable calls, the LLM part is required to return information in the format of a JSON dictionary. Additionally, each LLM part's prompt includes some examples, which contain inputs for certain scenarios and the corresponding expected outputs. If the input command does not contain the information of the keys of the output JSON dictionary, a default one will be filled in the dictionary. The parameters related to the GPT-4 API are all set to the official default values.

Note that, for supporting modification operations during multi-round commands, the 3D asset management agent, the vehicle motion agent, and the vehicle deleting agent have the ability to modify the information of already added or deleted cars.

\subsection{Reasoning Processes}
This section describes the natural language reasoning processes for the three cases presented in Section 5.2 of the main text.

\textbf{Mixed and complex command.} The initial input command is: \textit{"Remove all cars in the scene and add a Porsche driving the wrong way toward me fast. Additionally, add a police car also driving the wrong way and chasing behind the Porsche. The view should be moved 5 meters ahead and 0.5 meters above."} The command is decoupled by the project manager agent as following commands: 1.\textit{"Remove all cars."}; 2. \textit{"Add a Porsche driving the wrong way toward me fast."}; 3. \textit{"Add a police car also driving the wrong way and chasing behind the Porsche."}; 4. \textit{"The view should be moved 5 meters ahead and 0.5 meters above."}. The \textit{"Remove all cars."} command is distributed to the vehicle deleting agent, and then the agent finds the 3D boxes of all cars and applies the inpainting function for the removal operation. \textit{"Add a Porsche driving the wrong way toward me fast."} command is distributed to the 3D asset management agent for selecting the proper 3D asset. This command will also be distributed to the vehicle motion agent, which utilizes the key information in the command including "wrong way", "toward me" and "fast" to choose the appropriate start and end points and generate the motion with the motion generation function. \textit{"Add a police car also driving the wrong way and chasing behind the Porsche."} command will also be executed in the same way as the former operation. This command mentions the information of the added car, and the added car's information has been memorized by the project manager. This information is offered to the vehicle motion agent for determining the added police car's location. \textit{"The view should be moved 5 meters ahead and 0.5 meters above."} command is distributed to the view adjustment agent. The view adjustment agent returns the adjustment information of extrinsic as configuration, and calls the function to change the extrinsics to achieve view adjustment. Finally, background rendering and foreground rendering agents are required to generate the background and foreground results according to the information returned by the other agents, and the results are composed as the final outputs.

\textbf{Highly abstract command.} The initial input command is: \textit{"Create a traffic jam."} The project manager agent analyzes the command and decouples it as multiple repeats of car addition. These addition commands are processed by the 3D asset management agent and vehicle motion agent successively and are rendered by the foreground rendering agent. Combined with the rendered results from the background rendering agent, we can get the final outputs.

\textbf{Multi-round command.} The first initial command is: \textit{"Ego vehicle drives ahead slowly. Add a car to the close front that is moving ahead.”} The command is decoupled by the project manager agent as 1: \textit{"Ego vehicle drives ahead slowly."}; 2: \textit{"Add a car to the close front that is moving ahead."}. The first sub-command is distributed to view the adjustment agent, and the agent generates the extrinsics that represent moving ahead slowly. The second sub-command is executed as the process introduced above. 

The second initial command is: \textit{"Modify the added car to turn left. Add a Chevrolet to the front of the added car. Add another vehicle to the left of the added Mini driving toward me."} The command is decoupled by the project manager agent as 1: \textit{"Modify the added car to turn left."}; 2: \textit{"Add a Chevrolet to the front of the added car."}; 3: \textit{"Add another vehicle to the left of the added Mini driving toward me."} The first sub-command is distributed to the vehicle motion agent, which generates new motion based on the command for the determined added car. The following two sub-commands are executed in the same way as mentioned in the paragraphs above. Compositing the outputs of background rendering and foreground rendering agents can get the final outputs.


\section{Skydome Lighting Estimation Details}
\subsection{HDRI dataset}
We collect 449 high-quality outdoor panorama HDRIs from \href{https://polyhaven.com/hdris}{Poly Heaven Website}. These HDRIs are all licensed as CC0. We randomly selected 357 HDRIs for the training set and the remaining for the test set. A script for downloading these HDRIs will be available. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{imgs/sup_skydome1.jpg}
        \vspace{-3mm}
    \caption{LDR to HDR reconstruction network. We add an explicit spherical Gaussian lobe encoded attenuation to overcome the over-smoothness in the decoded HDR panorama. It effectively ensures that the sun's intensity significantly exceeds that of surrounding pixels, rendering strong shadow effects for inserted objects. }
    \label{fig:ldr_to_hdr}
    \vspace{-3mm}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{imgs/sup_skydome2.jpg}
    \vspace{-3mm}
    \caption{Reconstructing HDR skydome from multi-camera images. Training on HoliCity~\cite{zhou2020holicity} dataset.}
    \vspace{-3mm}
    \label{fig:predict_from_mc}
\end{figure*}

\subsection{LDR to HDR Skydome Reconstruction}
In this step, we utilize our HDRI dataset to train an LDR to HDR autoencoder with the aim of converting the skydome into a compact feature representation. We use the sRGB opto-electronic transfer function (also known as gamma correction) to get the LDR sky panorama, and follow ~\cite{wang2022neural} to transform the LDR sky panorama to 3 intermediate vectors, including the sky content vector $\mathbf{f}_{\rm content} \in \mathbb{R}^{64}$, the peak direction vector $\mathbf{f}_{\rm dir} \in \mathbb{R}^{3}$ and the intensity vector $\mathbf{f}_{\rm int} \in \mathbb{R}^{3}_{+}$. In the process of converting intermediate vectors into a reconstructed HDR sky panorama, we construct the peak direction map \(\mathbf{M}_{\rm dir}\), the peak intensity map \(\mathbf{M}_{\rm int}\) and the positional encoding map \(\mathbf{M}_{\rm pe}\).

Peak direction map (\(\mathbf{M}_{\rm dir}\)): For each pixel in \(\mathbf{M}_{\rm dir}\), we calculate the peak direction embedding. This calculation utilizes a spherical Gaussian lobe, formulated as \(\mathbf{M}_{\rm dir}(\mathbf{u}) = e^{100*(\mathbf{u}\cdot \mathbf{f}_{dir} -1)}\), where \(\mathbf{f}_{\rm dir}\) denotes the peak direction vector. This map is represented in  \(\mathbb{R}^{H \times W \times 1}\).

Peak intensity map (\(\mathbf{M}_{\rm int}\)): Each pixel in this map is determined based on its corresponding value in the peak direction map. Specifically, for a given direction \(\mathbf{u}\), if \(\mathbf{M}_{\rm dir}(\mathbf{u}) > 0.9\), then \(\mathbf{M}_{\rm int}(\mathbf{u})\) is assigned the value of \(\mathbf{f}_{\rm int}\). If not, \(\mathbf{M}_{\rm int}(\mathbf{u})\) is set to zero. This map is represented in  \(\mathbb{R}_{+}^{H \times W \times 3}\).

Positional encoding map (\(\mathbf{M}_{\rm pe}\)): This map encodes the direction vector of each pixel, determined through equirectangular projection, thus contributing to the accurate reconstruction of the HDR sky panorama. It is defined in  \(\mathbb{R}^{H \times W \times 3}\).

The input of the decoder $\mathbf{M}_{\rm input}$ is a concatenation of $\mathbf{M}_{\rm pe}, \mathbf{M}_{\rm dir}$ and $ \mathbf{M}_{\rm int}$. We use a 2D UNet to decode the concatenated input map to the HDR sky panorama. For sky content vector $\mathbf{f}_{\rm content}$, we use an MLP to increase its feature dimension, reshape it to a 2D feature map, and concatenate it with the intermediate features at the bottleneck of the UNet. This concatenated feature will be further decoded to the HDR sky panorama.

In the context of HDR imaging, the intensity of the peak often exhibits characteristics akin to an impulse response, displaying pixel values that are significantly elevated by orders of magnitude in comparison to adjacent pixels. This presents a substantial challenge for the decoder in accurately recovering these patterns. Thus, we design a residual connection to explicitly inject the peak intensity information into the final HDR sky panorama. Let \(\mathbf{M}_{\rm peak}\) be the product of \(\mathbf{M}_{\rm dir}\) and \(\mathbf{M}_{\rm int}\), representing an attenuation encoded by a spherical Gaussian lobe. In our design, we specifically substitute the decoded HDR sky panorama at the peak position with \(\mathbf{M}_{\rm peak}\). This substitution is applied where the value of \(\mathbf{M}_{\rm int}(\mathbf{u})\) is non-zero, ensuring that the peak position in the HDR sky panorama is accurately represented by \(\mathbf{M}_{\rm peak}\). This makes a significant difference between us and ~\cite{wang2022neural}. Accurate and strong peak intensity can generate very strong shadow effects, resulting in better rendering realism. See Figure ~\ref{fig:ldr_to_hdr}.

To train the LDR to HDR skydome reconstruction, we computer the ground truth peak direction \(\mathbf{f}_{\rm dir}^{\rm gt}\) and peak intensity \(\mathbf{f}_{\rm int}^{\rm gt}\) from the HDR ground-truth. During the network training process, we employ four losses for supervision. These losses are as follows: 
peak direction loss $L_{\rm dir}$, which measures the L1 angular error of the peak direction vectors;
peak intensity loss $L_{\rm int}$, which quantifies the log-encoded L2 error of the peak intensity vectors;
HDR reconstruction loss $L_{\rm hdr-recon}$, which evaluates the log-encoded L2 error between the reconstructed HDR output and the ground truth HDR data;
LDR reconstruction loss $L_{\rm ldr-recon}$, which is calculated as the L1 error between the input LDR sky panorama and the gamma-corrected HDR reconstruction. 

The total loss is $L_{\rm total} = \lambda_1 L_{\rm dir} + \lambda_2 L_{\rm int} + \lambda_3 L_{\rm hdr-recon} + \lambda_4 L_{\rm ldr-recon}$, where $\lambda_1=1, \lambda_2=0.1, \lambda_3=2$ and $\lambda_4=0.2$. 

Data augmentation methods, including rotation, flipping, exposure adjustment and white balance adjustment, are implemented to enrich the training data. Noticing a strong white balance inaccuracy (the color temperature is too high) in the image data from Waymo Open Dataset~\cite{sun2020scalability}, we augment the HDRI with corresponding white balance adjustment. The blue channel is randomly enlarged by 1.2-1.3 times, and the red channel is randomly reduced by 1.2-1.3 times. 



\subsection{Predict HDR Skydome from Multi-Camera Images}
This step involves estimating skydome lighting from multi-camera images collected by the vehicle. The core idea is to estimate intermediate features from multiple views and restore the skydome lighting using the well-trained HDR reconstruction decoding module. We emphasize the fusion of intermediate features from multiple cameras to get a complementary and comprehensive prediction for the skydome lighting.

Multi-camera image data will first go through a shared image encoder to predict the peak direction vector $\mathbf{f}_{\rm dir}^{(i)}$, the intensity vector $\mathbf{f}_{\rm int}^{(i)}$, and the sky content vector $\mathbf{f}_{\rm content}^{(i)}$ for each image $\mathcal{I}^{(i)}$, where $i$ is the camera index. For those vectors from $N$ cameras, we fuse all the features in the following strategy:

 We transform $\mathbf{f}_{\rm dir}^{(i)}, i=1,2,...,N$ to the front-facing view using their extrinsic parameters and averaged the rotated direction vector to $\bar{\mathbf{f}}_{\rm dir}$; we average $\mathbf{f}_{\rm int}^{(i)}, i=1,2,...,N$ to $\bar{\mathbf{f}}_{\rm int}$; we utilize the attention mechanism to fuse sky content vectors as $\bar{\mathbf{f}}_{\rm content} = \texttt{Attn(q, k, v)}$, where $\texttt{q} = \mathbf{f}^{(0)}_{\rm content}$, $\texttt{k} =\texttt{v} = \texttt{stack} (\{\mathbf{f}^{i}_{\rm content}\}_{i=0,1,...,N-1})$. Here index 0 refers to the first (front-facing) view image and $\texttt{Attn}(\cdot,\cdot,\cdot)$ the standard attention operator. Given $\bar{\mathbf{f}}_{\rm dir}$, $\bar{\mathbf{f}}_{\rm int}$, $\bar{\mathbf{f}}_{\rm content}$, we use the pre-trained decoding module from the previous stage to recover the fused intermediate vectors to HDR panorama. See Figure ~\ref{fig:predict_from_mc}.

Since there is no relevant panoramic data in the autonomous driving dataset for supervision, We use HoliCity~\cite{zhou2020holicity} to simulate multi-camera images.  Based on the arrangement and FOV of the three forward-facing cameras on the Waymo vehicle~\cite{sun2020scalability}, we cropped the corresponding image from the HoliCity panorama as the model inputs. To supervise the learning of the image encoder, we use the LDR to HDR reconstruction network from the previous stage to generate pseudo peak intensity vector GT, peak direction vector GT, sky content vector GT, and HDR skydome GT. 

We apply five losses to supervise the network during training. These losses are as follows: the peak direction loss $L_{\rm dir}$, which measures the L1 angular error of the fused peak direction vector; the peak intensity loss $L_{\rm int}$, which calculates the log-encoded L2 error of the fused peak intensity vectors; the sky content loss $L_{\rm content}$, which evaluates the L1 error of the fused sky content vectors; the HDR reconstruction loss $L_{\rm hdr-recon}$ with log-encoded L2 error; the LDR reconstruction $L_{\rm ldr-recon}$ with L1 error. 

The total loss is $L_{\rm total} = \lambda_1 L_{\rm dir} + \lambda_2 L_{\rm int} + \lambda_3 L_{\rm content} + \lambda_4 L_{\rm hdr-recon} + \lambda_5 L_{\rm ldr-recon}$, where $\lambda_1=0.5, \lambda_2=0.25, \lambda_3=0.005, \lambda_4=0.1$ and $\lambda_5=0.2$. 


\section{3D Asset Bank}
To ensure ease of access and modification of 3D assets, we normalize our Blender models within their Blender files using the following procedure:

\begin{enumerate}
    \item We ensure that the model has accurate physical dimensions in the unit of meter.
    
    \item The origin of the car model is set at the middle of the bottom of the car. We position the model at the center of the world coordinate system, ensuring that the car model's origin aligns with the origin of the world coordinate system. The car is oriented to face the positive direction of the x-axis.

    \item We uniformly apply the \texttt{Principled BSDF} material to the car body, and name the material "car\_paint". Prompt that changes the asset's color will affect the "Base Color" attribute of the \texttt{Principled BSDF} node.

    \item We use the \texttt{Join} operator to merge all meshes into one object. 

\end{enumerate}

Following the aforementioned approach, we normalize the Blender models collected from the Internet to continuously expand our 3D Asset Bank.

\section{Blender Rendering Details}
We fully implement the Blender rendering workflow using Python scripting, incorporating features such as alpha channel, depth channel, and shadow effect, \textbf{all achieved within a single rendering pass}.

\begin{enumerate}
    \item To get a transparent background, we first enable the \texttt{Render Properties - Film - Transparent} option.
    \item To get multiple rendering output, we enable the \texttt{Combined} pass, \texttt{Z} pass and \texttt{Shadow Catcher} pass in \texttt{View Layer Properties} panel.
    \item To render the shadow, we add a very large plane under the car and enable the plane's \texttt{Object Properties - Visibility - Mask - Shadow Catcher} option. 
    \item To obtain scene-related colored shadows, we construct the compositing node graph as Figure ~\ref{fig:blender}. This configuration generates the rendered image overlaid on the scene image, along with the accompanying depth information and mask of the vehicle and its corresponding shadow.
    \begin{figure}[t]
        \centering
        \includegraphics[width=\columnwidth]{imgs/blender_node.jpeg}
            \vspace{-3mm}
        \caption{Compositing node graph design in Blender~\cite{blender}}
        \label{fig:blender}
            \vspace{-3mm}
    \end{figure}
    \item Using depth information and mask, we can handle the occlusion relationship with the original objects in the scene. We also added a moderate amount of motion blur to the rendered car to match the background.
\end{enumerate}





\section{Motion Generation Details}
The vehicle motion agent creates the initial places and subsequent motions of vehicles following the requests commands. Existing vehicle motion generation methods cannot directly generate motion purely from text and the scene map. Here we elaborate on the details of our text-to-motion methods. Our method consists of two parts: 
vehicle placement to generate the starting points and vehicle motion planning to generate the subsequent motions.

\begin{figure}
    \centering
    \includegraphics[width=0.38\textwidth]{imgs/supp_placement.png}
    \caption{The neighboring area division for vehicle placement.}
    \label{fig:vehicle_placement}
    \vspace{-3mm}
\end{figure}

\subsection{Vehicle Placement}
We use the language command and the scene map to generate the initial position. The scene map $\mathcal{M}$ follows the lane map form $\mathcal{M}=\{\mathbf{n}_i,i=1,2,\cdots,m\}$, where $m$ is the number of lane nodes and the $i$th lane node $\mathbf{n}_i=(x_{\rm s},y_{\rm s},x_{\rm e},y_{\rm e},c_{\rm type})$ consists of lane starting position $(x_{\rm s},y_{\rm s})$, ending position $(x_{\rm e},y_{\rm e})$ and the lane type $c_{\rm type}$. The map range is cropped with the range of front 80m, left 20m and right 20m. Generally, we use the lane map from the ground-truth data. If the lane map does not exist, it is applicable to use a lane map estimation method like \cite{liao2022maptr,liao2023maptrv2} to obtain the lane map. 

Given the language command, the LLM first extracts key placement attributes, including vehicle number, distance range, relative direction with the observer and direction of driving, and crazy mode. With these attributes, the role function of placement begins to find suitable lane nodes from the scene map. Here we assume all the placed vehicles are on the centerline of the road. If the distance range $(d_{\rm min},d_{\rm max})$ is identified, the role function selects the lane centerline nodes according to their distance with the ego location. For the relative direction, we divide the ego neighboring area into 6 categories: front, left front, right front, left, right, and back, see Figure~\ref{fig:vehicle_placement} for illustration. For the direction of driving, we consider two types: driving close to the ego and driving away from the ego, which determines the left/right side of the vehicle on the road. The crazy mode, which is designed for non-compliant inverse driving behavior, is a bool variable. When it is true, we will inverse the direction of the map (swap the starting and ending point of each lane) for that vehicle to represent inverse driving. We select the matched lane node set and randomly select one lane node from the set. We also consider the conflict of placing vehicles by an iterative approach that incoming vehicles should not overlap with the existing vehicles. After obtaining lane nodes for every vehicle, we set the midpoint of the lane node to be the initial position of a vehicle and the direction of the lane to be the initial heading of the vehicle.

\subsection{Vehicle Motion Planning}
After obtaining the initial positions, we generate motions in two steps: plan the destination and plan the middle trajectory. We first extract movement attributes including speed, action, interval and time length. Notably, we divide actions into 5 categories: straightforward, turn left, turn right, park, and backward.  
To obtain the destination, if the action category is straightforward or park, and backward, we directly calculate a raw destination by assuming the car driving following a line with the target speed. Then we find the closest lane node with the raw destination to be the final destination.
If the action category is turning left or turning right, we select a set of nodes whose vertical distance with the initial line of heading is in a range (5m-30m) and fit the driving directions (the direction of the line should be away from the starting point). We randomly pick a lane node to be the destination. 

To plan the middle trajectory, we use an iterative adjustment approach to make the trajectory match with the map and avoid off-road driving. We first use one cubic Bezier curve to fit the overall trajectory with the condition of starting point, starting direction, ending point and ending direction. The cubic Bezier curve is formulated by
\begin{equation}
\begin{aligned}
    B(t) = & (1-t)^3P_0 + 3t(1-t)^2P_1 \\
    &+ 3t^2(1-t)P_2 + t^3P_3, t\in [0,1], 
\end{aligned}
\end{equation}
where $P_0,P_1,P_2,P_3 \in \mathbb{R}^2$ is the control points that can be solved by given starting point, starting direction, ending point and ending direction. Then to avoid off-road driving of the intermediate trajectory, we adjust the middle coordinate by replacing it with the closest lane node. We split the whole trajectory into two parts with the boundary of the middle coordinate and use one cubic Bezier curve to fit each split trajectory. We iteratively repeat the process to represent the planned trajectory by multiple cubic Bezier curves. Finally, to make the planned trajectory fit with vehicle dynamics, we use a trajectory tracking method in \cite{xu2023drl} as post-processing to revise the planned trajectory.





\section{Background rendering details}
\subsection{Dataset Selection}
For all Waymo Open Dataset~\cite{sun2020scalability} experiments, we use images captured from three frontal cameras. The details of selection are shown in Table~\ref{dataset}. There are 120 images in total for each scenerio.

\begin{table}[]
\centering
\scriptsize
\begin{tabular}{c|c}
\toprule
Sequence & Start Frame \\
\midrule
segment-10247954040621004675\_2180\_000\_2200\_000 & 0 \\
segment-13469905891836363794\_4429\_660\_4449\_660 & 40 \\
segment-14333744981238305769\_5658\_260\_5678\_260 & 40 \\
segment-1172406780360799916\_1660\_000\_1680\_000 & 50 \\
segment-4058410353286511411\_3980\_000\_4000\_000 & 90 \\
segment-10061305430875486848\_1080\_000\_1100\_000 & 30 \\
segment-14869732972903148657\_2420\_000\_2440\_000 & 0 \\
segment-16646360389507147817\_3320\_000\_3340\_000 & 0 \\
segment-13238419657658219864\_4630\_850\_4650\_850 & 0 \\
segment-14424804287031718399\_1281\_030\_1301\_030 & 60 \\
segment-15270638100874320175\_2720\_000\_2740\_000 & 60 \\
segment-15349503153813328111\_2160\_000\_2180\_000 & 100 \\
segment-15868625208244306149\_4340\_000\_4360\_000 & 110 \\
segment-16608525782988721413\_100\_000\_120\_000 & 10 \\
segment-17761959194352517553\_5448\_420\_5468\_420 & 0 \\
segment-3425716115468765803\_977\_756\_997\_756 & 0 \\
segment-3988957004231180266\_5566\_500\_5586\_500 & 0 \\
segment-9385013624094020582\_2547\_650\_2567\_650 & 130 \\
segment-8811210064692949185\_3066\_770\_3086\_770 & 30 \\
segment-10275144660749673822\_5755\_561\_5775\_561 & 0 \\
segment-10676267326664322837\_311\_180\_331\_180 & 100 \\
segment-12879640240483815315\_5852\_605\_5872\_605 & 20 \\
segment-13142190313715360621\_3888\_090\_3908\_090 & 0 \\
segment-13196796799137805454\_3036\_940\_3056\_940 & 70 \\
segment-14348136031422182645\_3360\_000\_3380\_000 & 140 \\
segment-15365821471737026848\_1160\_000\_1180\_000 & 0 \\
segment-16470190748368943792\_4369\_490\_4389\_490 & 0 \\
segment-11379226583756500423\_6230\_810\_6250\_810 & 0 \\
segment-13085453465864374565\_2040\_000\_2060\_000 & 110 \\
segment-14004546003548947884\_2331\_861\_2351\_861 & 0 \\
segment-15221704733958986648\_1400\_000\_1420\_000 & 70 \\
segment-16345319168590318167\_1420\_000\_1440\_000 & 0 \\
\bottomrule
\end{tabular}
            \vspace{-3mm}
\caption{\small  Information on the selected and trimmed Waymo Open Dataset~\cite{sun2020scalability}. For each sequence, we select 40 frames starting from the Start Frame.  }
\label{dataset}
    \vspace{-3mm}
\end{table}

\begin{figure}
\centering 
\includegraphics[width=0.47\textwidth]{imgs/supp_compare.png} 
\vspace{-3mm}
\caption{\small Qualitative ablation of background rendering. (a) McNeRF w/o pose alignment.(b) McNeRF w/o exposure. (c) Full McNeRF. Last row: target images.}
\label{Fig:ablation} 
\vspace{-3mm}
\end{figure}

\subsection{Multi-Camera Alignment}
This section will introduce the details of our multi-camera alignment algorithm. Let $R_{C_i, t}$ and $T_{C_i, t}$ represents the camera $C_i$'s extrinsic matrix that aligned to vehicle's coordinates at timestamp $t$. $C_0$ is the front camera. The superscript $(V)$ and $(M)$ represents the original vehicle's coordinates in autonomous driving dataset and the coordinates under Metashape's unified space. Then the rotation $R_{C_i, t}$ and translation $T_{C_i, t}$ can be calculated as:
\begin{align*}
R_{C_i, t} &= R^{(V)}_{C_0, 0} (R^{(M)}_{C_0, 0})^{-1} R^{(M)}_{C_i, t} \\
T_{C_i, t} &= \frac{R^{(V)}_{C_0, 0} (R^{(M)}_{C_0, 0})^{-1} (T^{(M)}_{C_i, t} - T^{(M)}_{C_0, 0})}{S} + T^{(V)}_{C_0, 0}, \\
\end{align*}
where $S=\frac{T^{(M)}_{C_0, 1} - T^{(M)}_{C_0, 0}}{T^{(V)}_{C_0, 1} - T^{(V)}_{C_0, 0}}$ is a scaling factor that ensures the aligned space has the same unit length as the real world.


\section{Supplymentary Experiments}

\subsection{Qualitative Ablation Study of Background Rendering}
Figure \ref{Fig:ablation} illustrates the effects of the ablation study on background rendering. It is evident that in the absence of pose adjustment, the rendered results exhibit significant blur and anomalies. Without the intervention of exposure adjustments, there are noticeable changes in brightness at the junctions of different cameras, particularly in the sky. McNeRF, however, successfully avoids these two issues and achieves the optimal rendering outcomes.

\begin{figure*}
\centering 
\includegraphics[width=0.99\textwidth]{imgs/supp_occlusion.png} 
\vspace{-3mm}
\caption{\small Qualitative result of occlusion postprocess and the color control for added car.}
\label{Fig:occlusion} 
\end{figure*}
\subsection{Occlusion with Depth Test}
During the process of adding vehicles, there may be instances of occlusion. For occlusions among multiple vehicles to be added, Blender considers this issue during the rendering process. Therefore, we only need to focus on the occlusion between the foreground vehicles and the background objects. The most straightforward method to handle occlusion is determined by the depth map of the foreground and background, respectively. The depth maps of both the foreground and background could be used to choose for each pixel with the lesser depth to be displayed in the front, while the one with greater depth is occluded. However, accurately estimating the background's depth map directly is challenging. The point cloud data in autonomous driving datasets is too sparse, and the depth maps obtained through depth completion are also sparse and excessively noisy, making them unsuitable for pixel-level accuracy in practical use. Here, we combine the sparse depth data from point clouds with the object segmentation method SAM\cite{kirillov2023segment}. SAM can achieve pixel-level accuracy in segmentation results at the image level, without extra finetuning. We first use SAM to obtain different patches in the background image, then identify patches that overlap with the foreground objects. Using the sparse depth map derived from the point clouds, we calculate the average sparse depth within these patches as the depth of each patch. Since the segmentation results of patches often represent a complete instance, and occlusion occurs between instances, it is reasonable to calculate the depth for the entire instance represented by a patch. Subsequently, we create the background's depth map from the depths of these patches and perform occlusion calculations with the depth map rendered for the foreground, presenting each pixel with the lesser depth to finalize the occlusion computation. The results of the occlusion calculation, as shown in Fig. \ref{Fig:occlusion}, illustrate that the added vehicles are occluded by those with shallower depths. This figure also displays the adjustment of the added vehicles' colors.

\begin{figure*}
\centering 
\includegraphics[width=0.99\textwidth]{imgs/supp_obstacles.png} 
\vspace{-3mm}
\caption{\small Qualitative results of rare cases simulation.}
\label{Fig:obstacles} 

\end{figure*}

\subsection{Rare Cases Simulation}
Leveraging diverse external digital assets, ChatSim can simulate rare and challenging-to-collect real-world scenarios within reconstructed existing scenes. Figure \ref{Fig:obstacles} demonstrates ChatSim's ability to emulate rare cases by placing uncommon elements like bulldozers, isolation piers, fences, excavators, and other infrequently encountered situations in reconstructed scenes. This capability enables ChatSim to create rare digital twins for existing collected data, thus fulfilling the need for these specific scenarios.

\begin{table}[]
\centering
\begin{tabular}{c|ccc}
\toprule
Simulation data & AP30            & AP50            & AP70            \\ \hline
            0               & 0.1263          & 0.0366          & 0.0034       \\
            600             & 0.1910          & 0.0878          & 0.0153       \\
            1000            & \textbf{0.2074} & \textbf{0.0930} & \textbf{0.0189} \\
            2200            & 0.2064          & 0.0900          & 0.0182      \\ 
            \hline
\end{tabular}
            \vspace{-3mm}
\caption{Comparison of detection model’s performance with different number of data simulated by ChatSim}
\label{tab:augmentation_2}
\vspace{-3mm}
\end{table}

\subsection{Supplementary 3D Detection Augmentation Experiment}

We conducted 3D detection augmentation experiments under a new setting: we fixed the real data amount from the original dataset at 4200 frames and augmented it with varying quantities of simulation data generated by ChatSim. We continued to use Lift-Splat~\cite{philion2020lift} as the detection model, with results shown in Table \ref{tab:augmentation_2}. It is observed that the use of simulation data significantly enhances the performance of the 3D detection task. As the amount of simulation data increases, the final performance tends to stabilize after a certain point of improvement.


% \section{User Study Details}
% \textbf{Motion experiment user study.} We generate 35 different motions for our motion generation method and the two baselines with specific action control and visualize the motion and map. The 12 users are required to judge if the visualization of motion satisfies the action and if the motion is within the road boundary. 
